Blockchain Abstract Data Type

The presented work continues the line of recent distributed computing communityefforts dedicated to the theoretical aspects of blockchains. This paper is the rst tospecify blockchains as a composition of abstract data types all together with a hierarchyof consistency criteria that formally characterizes the histories admissible for distributedprograms that use them. Our work is based on an original oracle-based constructionthat, along with new consistency deffnitions, captures the eventual convergence processin blockchain systems. The paper presents as well some results on implementability ofthe presented abstractions and a mapping of representative existing blockchains fromboth academia and industry in our framework.

==> corePaper.tex <==
% !TeX root = mainDISC18.tex


\section{Preliminaries on shared object specifications based on Abstract Data Types}
\label{sec:paper-adt}

The basic idea underlying the use of abstract data types is to specify shared objects using two complementary facets~\cite{matthieu-book}: a sequential specification that describes the semantics of the object, and a consistency criterion over concurrent histories, i.e. the set of admissible executions in a concurrent environment. In this work we are interested in consistency criteria achievable in a distributed environment in which processes are sequential and communicate through message-passing.

%\subsection{Abstract Data Type (ADT)}
%\label{sec:abstract-data-type}

\subsection{Abstract Data Type (ADT)}
The model used to specify an abstract data type is a form of transducer, as Mealy's machines, accepting an infinite but countable number of states. The values that can be taken by the data type are encoded in the abstract state, taken in a set $Z$. We refer by \(\xi_0 \in Z\) the initial state of the ADT. It is possible to access the object using the symbols of an input alphabet $A$. Unlike the methods of a class, the input symbols of the abstract data type do not have arguments. Indeed, as one authorizes a potentially infinite set of operations, the call of the same operation with different arguments is encoded by different symbols. An operation can have two types of effects. First, it can have a side-effect that changes the abstract state, the corresponding transition in the transition system being formalized by a transition function $\tau$. Second, operations can return values taken in an output alphabet $B$, which depends on the state in which they are called and an output function $\delta$. For example, the pop operation in a stack removes the element at the top of the stack and returns that element (its output).  In the following, an abstract data type refers to a 6-tuple $T=\langle A,B, Z, \xi_0, \tau, \delta \rangle $. The formal definition can be found in \cite{BTADT2018TR}.

\subsection{Sequential specification of an ADT}
An abstract data type, by its transition system, defines the sequential specification of an object. That is, if we consider a path that traverses its system of transitions, then the word formed by the subsequent labels on the path is part of the sequential specification of the abstract data type, i.e. it is a sequential history. A sequential history of an ADT \(T\) refers to a sequence \((\sigma_i)_{i\geq 0}\) (finite or not) of operations leading state of \(T\) to evolve according to its specification. The formal definition of a sequential specification appears in \cite{BTADT2018TR}.

\subsubsection{Concurrent histories of an ADT}

Concurrent histories are defined considering asymmetric event structures, i.e., partial order relations among events executed by different processes. 
A set of processes \(V\) invoking operations of an ADT defines a concurrent history. Operations are not executed instantaneously. Given an operation \(o \in \Sigma = A \cup ( A \times B)\), we denote by $e_{inv}(o)$ the \(o\) invocation event and by $e_{rsp}(o)$ the corresponding response event. In addition, we denote by $e_{rsp}(o):x$ the returned value associated to the response event  $e_{rsp}(o)$.
In the following \(E\) represents the set of events and \(\Lambda\) is the  function which associates events to the operations in $\Sigma$.
Given a process \(p \in V\) and two operations \(o_1, o_2\), if \(p\) executes \(o_1\) before \(o_2\), that is if \(e_{rsp}(o_1)\) appends before \(e_{inv}(o_2)\), we say that \(o_1\) precedes \(o_2\) in \emph{process order}, denoted by \(o_1 \mapsto o_2\). 
Given two events \(e, e^\prime \in E\), we say that \(e\) precedes \(e^\prime\)  in \emph{operation order}, denoted by \(e \prec e^\prime\), if either \emph{(i)} $e$ is an operation invocation and $e'$ is the response for the same operation, or \emph{(ii)}  $e'$ is the invocation of an operation occurred at time $t'$ and $e$ is the response of another operation occurred at time $t$ with $t < t'$. %The order  $\prec $ is called the operation order.
Finally, for any couple of events \((e,e^\prime) \in E^2\) with $e \neq e'$, we say that \(e\) precedes \(e^\prime\) in \emph{program order}, denoted by $e \nearrow e'$, if $e \mapsto e'$ or $e \prec e'$. 
These asymetric event structures allow us to define a concurrent history of an ADT  T =$\langle A, B, Z, \xi_0, \tau, \delta \rangle$ as a 6-tuple $H=\langle \Sigma, E, \Lambda, \mapsto, \prec, \nearrow \rangle$. More details are given in \cite{BTADT2018TR}. 

\subsubsection{Consistency criterion}
A consistency criterion characterizes which concurrent histories are admissible for a given abstract data type. It  can be viewed as a function that associates a concurrent specification to abstract data types. 
Given a consistency criterion \(C\), an algorithm $A_T$ implementing the ADT $T$  %\in \mathcal{T}$ 
is $C$-consistent if all the operations terminate and all the admissible executions are $C$-consistent, i.e. they satisfy \(C\).



\section{BlockTree and Token oracle ADTs}
\label{sec:blocktr-token-oracle}


In this section we present the BlockTree and the token Oracle ADTs along with consistency criteria. 

\subsection{BlockTree ADT}
\label{subsec:blocktree}
We formalize the data structure implemented by blockchain-like systems as a \emph{directed rooted tree} $bt=(V_{bt},E_{bt})$
%, where each vertex of the BlockTree is a \emph{block},  and in which all edges point backward to the root, the genesis block. This data structure is called a \emph{BlockTree}. 
called \emph{BlockTree}. Each vertex of the BlockTree is a \emph{block} and any edge points backward to the root, called \emph{genesis block}.
The height of a block refers to its distance to the root. By convention, the root of the BlockTree is denoted by \(b_0\). Only block satisfying  some validity predicate $P$ can appear in the BlockTree. Predicate $P$ is application dependent. Predicate $P$ mainly abstracts the creation  process of a block, which may fail or successfully terminate. For instance, in Bitcoin, a block is considered valid if it can be connected to the current blockchain and does not contain double-spending transactions. 

In the following, we represent by $\mathcal{B}$  a countable and non empty set of blocks and by $\mathcal{B'}\subseteq \mathcal{B}$ a countable and non empty set of valid blocks, i.e.,  $\forall b \in \mathcal{B'}$, $P(b)\Leftrightarrow \top$.  By assumption $b_0 \in \mathcal{B'}$; We also denote by $\mathcal{BC}$ a countable non empty set of blockchains, where a blockchain is a path from a leaf of $bt$ to $b_0$. A blockchain is denoted by $bc$. Finally, $\mathcal{F}$ is a countable non empty set of selection functions, $f \in \mathcal{F} : \mathcal{BT} \rightarrow \mathcal{BC}$;  $f(bt)$ selects a blockchain $bc$ from the BlockTree $bt$ (note that $b_0$ is not returned) and if $bt=b_0$ then $f(b_0)=b_0$. This reflects for instance the longest chain or the heaviest chain used in some blockchain implementations. The selection function $f$ and the predicate $P$ are parameters of the ADT which are encoded in the state and do not change over the computation.
%
The following notations are used: $\{b_0\}^\frown {f(bt)}$ represents the concatenation of $b_0$ with the blockchain of $bt$; and  $\{b_0\}^\frown {f(bt)}^ \frown \{b\}$ represents  the concatenation of $b_0$ with the blockchain of $bt$  and a block $b$.


\subsubsection{Sequential specification of the BlockTree}
\label{sec:blocktr-sequ-spec}

The sequential specification of the BlockTree is defined as follows.

\begin{definition}[BlockTree ADT ($BT$-$ADT$)]
	
	The BlockTree Abstract Data Type 
	is the 6-tuple 
	BT-ADT=$\langle A=\{ {\sf append}$($b$)$, {\sf read}$()$: 
	b \in \mathcal{B}\}, B= \mathcal{BC}\cup\{ {\sf true},{\sf false}\}, Z= \mathcal{BT} \times \mathcal{F} \times (\mathcal{B} \rightarrow \{ {\sf true},{\sf false}\}) $, $\xi_0 = (bt^0, f), \tau, \delta \rangle$, where the transition function $\tau:Z \times A \rightarrow Z$ is defined by
	\[
	\tau((bt,f,P), {\sf read}())= (bt,f,P)~;~~ \tau((bt,f,P), {\sf append}(b))=\begin{cases}(\{b_0\}^\frown {f(bt)}^ \frown \{b\},f,P)  \textnormal{ if } b\in \mathcal{B'} \\ (bt,f,P) \textnormal{ otherwise}\end{cases}
	\]
	\noindent
	and the output function $\delta:Z \times A \rightarrow B$ is defined by
	\[
	\delta((bt,f,P), {\sf append}(b))=\begin{cases}
	\textnormal{{\sf true} if } b \in \mathcal{B'} \\ 
	\textnormal{{\sf false} otherwise}
	\end{cases}
	;~~ 
	\delta((bt,f,P), {\sf read}())=\begin{cases}
	\{b_0\} \textnormal{ if } bt=bt_0 \\
	\{b_0\}^\frown f(bt) \textnormal{ otherwise}
	\end{cases}
	\]
\end{definition}

The semantic of the {\sf read} and the {\sf append} operations directly depends on the selection function $f \in \mathcal{F}$. In this work we let this function generic to suit the different blockchain implementations. 


\begin{figure}
	\begin{tikzpicture}[->, auto]
	\tikzset{stato/.style={draw,circle, node distance=4.5cm}}
	\tikzset{dettaglio/.style={black!70}}
	\tikzset{blocco/.style={
			circle,
			inner sep=1pt,
			thick,
			align=center,
			draw=gray,
		}
	}
	
	\node[stato] (0) at (0,0) {$\xi_0 $};
	
	\node[dettaglio, below of=0] (s0) {$\xi_0 = \{$
		\begin{tikzpicture}[scale=0.8, every node/.style={scale=0.8}]	
		\node  [blocco] (i11) at (0.5,3)  {\scriptsize $b_0$};	
		\end{tikzpicture}
		$, f,P\}$};
	
	
	\node[stato, right of=0] (1) {$\xi_1$}; 
	\node[dettaglio, below of=1] (s1) {$\xi_1= \{$			
		\begin{tikzpicture}[scale=0.8, every node/.style={scale=0.8}]	
		\node  [blocco] (i11) at (0.5,3)  {\scriptsize $b_0$};
		\node  [blocco]  (i12) at (1.2,3) {\scriptsize $b_1$};
		\draw[<-] (i11) edge (i12)  ;
		\end{tikzpicture}
		$, f ,P\}$};
	
	\path (0) edge [bend left] node[align=center] {\scriptsize {\sf append}$ (b_1)/ {\sf true}$ \\ {\scriptsize{\bf if } $b_1 \in \mathcal{B'} $}} (1);
	\path (0) edge [loop left] node[align=center] {\scriptsize {\sf append}$( b_3)/ {\sf false}$ \\ {\scriptsize{\bf if } $b_3 \notin \mathcal{B'} $}} (0);	
	
	
	\node[stato, right of=1] (2) {$\xi_2$}; 
	\node[dettaglio, below of=2] (21) {$\xi_2= \{$
		\begin{tikzpicture}[scale=0.8, every node/.style={scale=0.8}]
		\node  [blocco] (i11) at (0.5,3)  {\scriptsize $b_0$};
		\node  [blocco]  (i12) at (1.3,3.2) {\scriptsize $b_1$};
		\node [blocco] (i13) at (1.3,2.7) {\scriptsize $b_2$};
		\draw[<-] (i11) edge (i12) (i11) edge (i13) ;
		\end{tikzpicture}
		$, f ,P\}$};	
	
	\path (1) edge [bend left] node[align=center] {\scriptsize {\sf append}$(b_2)/ {\sf true}$ \\ {\scriptsize{\bf if } $b_2 \in \mathcal{B'} $}} (2);
	\path (1) edge [loop right] node[align=center] {\scriptsize {\sf append}$(b_3)/ {\sf false}$ \\ {\scriptsize{\bf if } $b_3 \notin \mathcal{B'} $}} (1);
	
	
	\path (1) edge [loop above] node[align=center] {\scriptsize {\sf read}$()/ {b_0 ^\frown b_1}$} (1);	
	\path (2) edge [loop above] node[align=center] {\scriptsize {\sf read}$()/ {b_0 ^\frown b_2}$} (2);		
\end{tikzpicture}
\caption{A possible path of the transition system defined  by the BT-ADT. We use the following syntax on the edges: {\sf operation}/{\sf output}.}\label{fig:BT-ADT}
\end{figure}




\subsubsection{Concurrent histories  of a BT-ADT and consistency criteria}
\label{sec:conc-spec-bt}
A  $BT$-$ADT$ consistency  criterion is a function that returns the set of concurrent histories admissible for a BlockTree abstract data type.  We define two $BT$ consistency criteria:  \emph{BT Strong consistency} and \emph{BT Eventual consistency}. For ease of readability, we employ the following notations:
\begin{itemize}
	\item $E(a^*,r^*)$ refers to an infinite set containing an infinite number of {\sf append}$()$ and {\sf read}$()$ invocation and response events. Similarly, $E(a,r^*)$ refers to an infinite set containing {\em (i)} a finite number of {\sf append}$()$ invocation and response events and {\em (ii)} an infinite number of {\sf read}$()$ invocation and response events;
	\item ${\sf score}: \mathcal{BC}\rightarrow \mathbb{N}$ denotes a monotonically increasing deterministic function that takes as input a blockchain $bc$ and returns a natural number $s$ as score of $bc$, which can be the height, the weight, etc. Informally we refer to such value as the score of a blockchain; by convention we refer to the score of the blockchain uniquely composed by the genesis block as $s_0$, i.e. ${\sf score}(\{b_0\})=s_0$. Increasing monotonicity means that ${\sf score}(bc^\frown \{b\}) > {\sf score}(bc)$; 
	\item ${\sf mcps}: \mathcal{BC} \times \mathcal{BC} \rightarrow \mathbb{N}$ is a function that given two blockchains $bc$ and $bc'$ returns the score of the maximal common prefix of $bc$ and $bc'$;
	\item $bc \sqsubseteq bc^\prime$ iff $bc$ prefixes $bc^\prime$.
\end{itemize}

We now present the BT Strong consistency criterion. Informally it says that any two {\sf read}() operations return blockchains such that one is the prefix of the other. This is formalized through the following four properties. 


The Block validity property imposes that each block in a blockchain returned by a {\sf read}$()$ operation is \emph{valid} (i.e., satisfies predicate $P$) and has been inserted in the BlockTree with the {\sf append}$()$ operation. Formally,
\begin{definition}[Block validity] $\forall e_{rsp}(r) \in E, \forall b \in e_{rsp}(r):bc, b \in \mathcal B' \wedge \exists e_{inv}({\sf append}(b)) \in E, e_{inv}(append(b)) \nearrow e_{rsp}(r)$	
\end{definition}
The Local monotonic read property states that, given the sequence of {\sf read}$()$ operations at the same process, the score of the returned blockchain never decreases; Formally,
\begin{definition}[Local monotonic read] $\forall e_{rsp}(r), e_{rsp}(r') \in E^2, \text{ if } e_{rsp}(r) \mapsto e_{inv}(r'), \text{ then } \\{\sf score}(e_{rsp}(r):bc)\leq {\sf score}(e_{rsp}(r'):bc')$
\end{definition}
The Strong prefix property says  that for each pair of read operations, one of the returned blockchains is a prefix of the other returned one. Formally, 
\begin{definition}[Strong prefix] $\forall e_{rsp}(r), e_{rsp}(r') \in E^2,  (e_{rsp}(r'):bc' \sqsubseteq e_{rsp}(r):bc) \vee (e_{rsp}(r):bc \sqsubseteq e_{rsp}(r'):bc')$
\end{definition}
Finally, the Ever growing tree states that scores of returned blockchains eventually grow. More precisely, let $s$ be the score of the blockchain returned by a read response event $r$ in $E(a^*,r^*)$, then for each {\sf read}$()$ operation $r$, the set of {\sf read}$()$ operations $r'$ such that $e_{rsp}(r)\nearrow e_{inv}(r')$ that do not return blockchains with a score greater than $s$ is finite. Formally, 
\begin{definition}[Ever growing tree] $\forall e_{rsp}(r)  \in E(a^*,r^*), s={\sf score}(e_{rsp}(r):bc)\text{ then} \\ |\{ e_{inv}(r') \in  E \mid e_{rsp}(r) \nearrow e_{inv}(r'), {\sf score}(e_{rsp}(r'):bc')\leq s \}| <\infty$
\end{definition}

\begin{definition}[BT Strong  Consistency criterion $SC$]
	A concurrent history $H=\langle \Sigma, E, \Lambda, \mapsto, \prec, \nearrow \rangle$ of the system that uses a BT-ADT verifies the BT Strong Consistency criterion if the Block validity, Local monotonic read, Strong prefix and the Ever growing tree properties hold.
\end{definition}


We now present a weaker version of $SC$ introducing the BT Eventual consistency criterion. Informally, the BT Eventual consistency criterion says that eventually any two {\sf read}() operations return blockchains  that share the same prefix, which differs from the BT Strong consistency criterion by the Eventual prefix property. This property says that for each blockchain returned by a {\sf read}$()$ operation with $s$ as score, then eventually all the {\sf read}$()$ operations will return blockchains sharing the same maximum common prefix at least up to $s$. Say differently, let $H$ be a history with an infinite number of {\sf read}$()$ operations, and let $s$ be the score of the blockchain returned by a read $r$, then the set of {\sf read}$()$ operations $r'$, such that $e_{rsp}(r)\nearrow e_{inv}(r')$, that do not return blockchains sharing the same prefix at least up to $s$ is finite.  We formalise this notion as follows:

\begin{definition}[Eventual prefix property]\label{def:eventual=preficx}
	Given a concurrent history $H=\langle \Sigma, E(a,r^*), \Lambda, \mapsto, \prec, \nearrow \rangle$ of the system that uses a BT-ADT, we denote by \(s\), for any {\sf read} operation \(r \in \Sigma\) such that \(\exists e \in E(a,r^*), \Lambda(r) = e\), the score of the returned blockchain, \emph{i.e.}, \(s={\sf score}(e_{rsp}(r):bc)\).
	We denote by \(E_{r}\) the set of response events of read operations that occurred after \(r\) response, \emph{i.e.} \(E_{r} = \{ e \in E \mid \exists r^\prime \in \Sigma, r^\prime={\sf read}, e=e_{rsp}(r^\prime) \wedge e_{rsp}(r) \nearrow e_{rsp}(r')  \}\). Then, H satisfies the Eventual prefix property if for all {\sf read()} operations \(r \in \Sigma\)  with score $s$,  \[
	| \{ (e_{rsp}(r_h), e_{rsp}(r_k)) \in E_{r}^2 | h\neq k, {\sf mpcs}(e_{rsp}(r_h):bc_h, e_{rsp}(r_k):bc_k) < s \} | < \infty
	\]
\end{definition}

% The Eventual prefix property captures the fact that two or more concurrent blockchains can co-exist in a finite interval of time, but that eventually all the participants adopts a same branch for each cut of the history. This cut of the history is defined by a read that picks up a blockchain with a given score.  


\begin{definition}[BT Eventual consistency criterion  $E C$]
	A concurrent history $H=\langle \Sigma, E, \Lambda, \mapsto, \prec, \nearrow \rangle$ of the system that uses a BT-ADT verifies the \emph{BT Eventual consistency criterion} if it satisfies the Block validity, Local monotonic read, Ever growing tree, and the Eventual prefix properties.
\end{definition}


\subsubsection{Relationships between Eventual Consistency (EC) and Strong Consistency(SC).}

Let us denote by 
$\mathcal{H}_{E C} $ and by $\mathcal{H}_{SC} $ the set of histories satisfying respectively the $E C$ and the $SC$ consistency criteria.  


\begin{theorem}\label{th:strongImpliesEventualM}
	Any history $H$ satisfying $SC$ criterion satisfies $E C$  and $ \exists H$ satisfying  $E C$ that does not satisfy $SC$, i.e.,  
	$\mathcal{H}_{SC} \subset \mathcal{H}_{E C}$.
\end{theorem}

The proof of the Theorem and an illustration showing a BT Eventual Consistent history which is not Strong Consistent are proposed in \cite{BTADT2018TR}.

Let us remark that the BlockTree allows at any time to create a new branch in the tree, which is called a \textit{fork} in the blockchain literature. Moreover, an append is successful only if the input block is valid with respect to a predicate. This means that histories with no append operations are trivially admitted. 
In the following we introduce a new abstract data type called Token Oracle that when combined with the BlockTree will help in \emph{(i)} validating blocks and \emph{(ii)} controlling forks. In the following we introduce the Token Oracle  and then we define the properties on the BlockTree augmented with the Token Oracle.

\subsection{Token oracle $\Theta$}\label{sec:oracle}

The Token Oracle $\Theta$ aims at capturing the fact that processes can only insert valid blocks in the BlockTree and at  controling  the number of concurrent valid blocks that can be appended to a valid block in the BlockTree structure. This is provided by two operations of $\Theta$, namely the {\sf getToken()} and the {\sf consumeToken()} operations. Suppose  that process $i$ wishes to append its new block $b_\ell$ to the (valid) block $b_h$, where $b_h$ is the leaf of a blockchain already in the BlockTree structure. Process $i$ invokes {\sf getToken}$(b_h,b_\ell)$ operation. If $\Theta$  decides to provide the token, then {\sf getToken}$(b_h,b_\ell)$ returns $b_{\ell}^{tkn_{h}}$,   $\bot$ otherwise. Note that by definition $b_{\ell}^{tkn_{h}}\in \mathcal{B'}$.  Superscript ${tkn_{h}} $ means that $i$ receives a token from $\Theta$ to try to append its block $b_\ell$ to $b_h$. Once process $i$ has received token $tkn_{h}$, it asks $\Theta$ the right to append its valid block  $b_{\ell}^{tkn_{h}}$ to $b_h$  by invoking the {\sf consumeToken($b_{\ell}^{tkn_{h}}$)} operation. A maximal number $k$ of tokens are associated to each (valid) block in the BlockTree structure, and each token can be consumed only once. If there are $k$ valid blocks already appended to $b_h$ then {\sf consumeToken($b_{\ell}^{tkn_{h}}$)} does not allow the consumption of the token, otherwise $i$ is allowed to append its valid block to $b_h$ (we say that $i$ consumes its token for $b_h$) and the set of consumed tokens for $b_h$ is incremented with $b_{\ell}^{tkn_{h}}$. In any case, the operation returns the set containing all the tokens consumed for $b_h$. This allows to announce decided tokens in the system \cite{AM2017}, which is the key to endow Consensus synchronization power as showed in Theorem \ref{t:consensusOracleReduction}. 


We specify two token oracles, which differ in the way tokens are managed. 
The first oracle, called  {\em prodigal} and denoted by $\Theta_P$, has no upper bound on the number of tokens consumed for an object (i.e., $k=\infty$). This oracle, when combined with the BlockTree abstract data type, will only help in validating blocks. 
The second oracle, called {\em frugal}, and denoted by $\Theta_F$, manages tokens in a more controlled way to guarantee that no more than $k$ processes can consume a token for a given block, i.e., no more than $k$ forks can occur on a given block in the BlockTree. 

For both oracles, when {\sf getToken}$(b_h,b_\ell)$ operation is invoked, the oracle provides a token with a certain probability $p_{\alpha_i}>0$ where  $\alpha_i$ is a \say{merit} parameter characterizing  the invoking process $i$.~\footnote{The merit parameter can reflect for instance the hashing power of the invoking process.}
Note that the oracle knows $\alpha_i$ of the invoking process $i$, which might be unknown to the process itself. For each merit $\alpha_i$, the state of the token oracle embeds an infinite tape where each cell of the tape contains either $tkn$ or $\bot$. Since each tape is identified by a specific $\alpha_i$ and $p_{\alpha_i}$,  we assume that each tape contains a pseudorandom sequence of values in $\{tkn,\bot\}$ depending on $\alpha_i$.~\footnote{We assume a pseudo-random sequence mostly indistinguishable from a Bernoulli sequence  consisting of a finite or infinite number of independent random variables $X1, X2 , X3, \dots $ such that \emph{(i)}  for each $k$, the value of $X_k$ is either $tkn$ or $\bot$; and \emph{(ii)} $\forall X_k$ the probability that $X_k=tkn$ is $p$.}
%~\footnote{We assume that each tape is a sequence of independent Bernouilli trials with success probability \(p_{\alpha_i}\), that is, the \(k\)-th cell of the tape contains \(X_k^{\alpha^i}=tkn\) with probability \(p_{\alpha_i}\) or \(\bot\) with probability \(1-p_{\alpha_i}\). As a consequence, given \(\ell > 0\), the cell \(n\geq 0\) contains the \(\ell\)-th token of the tape with probability \( {n \choose \ell} p_{\alpha_i}^\ell (1-p_{\alpha_i})^{n-\ell}\). This means that a process will get \(\ell\) tokens after a finite number of {\sf getToken} invokations with probability 1. This argument holds for any value of \(\alpha_i\). The sequence of values poped from the cells of the different tapes is thus a sequence of independent Bernouilli trials with different success probabilities. Similarly, the number of invokations of {\sf getToken} required to get the \(\ell\)-th token is almost surely finite as well.} 
When a {\sf getToken}$(b_h,b_\ell)$ operation is invoked by a process with merit $\alpha_i$, the oracle pops the first cell from the tape associated to $\alpha_i$, and a token is provided to the process if that cell contains $tkn$. 

Both oracles also enjoy an infinite array $K$ of sets, one for each block, which is populated each time a token is consumed for a specific block. When the set cardinality reaches $k$ then no more tokens can be consumed for that block. For a sake of generality, $\Theta_P$ is defined as $\Theta_F$ with $k=\infty$ while for $\Theta_F$ a predetermined $k \in \mathbb{N}$ is specified. \\

In Figure \ref{fig:Theta-ADT} is depicted a possible path of the transition system defined  by the $\Theta_F$ and  $\Theta_P$-ADTs. As we can see in the Oracle state there is $K$, an infinite array of sets where up to $k$ valid blocks are stored, along with infinite tapes, one for eache possible merit.  When a process with merit $\alpha_1$ invokes {\sf getToken}$(b_1,b_k)$ the first cell of $tape_{alpha_1}$ is popped, since it contains a token, then {\sf getToken}$(b_1,b_k)$ returns a valid block $b_k^{tkn_1}$. Afterwards, when {\sf consumeToken}$b_k^{tkn_1}$ is invoked, the Oracle checks if the cardinality of the set in $K[1]$ is strictly smaller than $k$ and if the block is valid. If both conditions hold then $K[1] \leftarrow K[1] \cup b_k^{tkn_1}$ (which means that $b_k$ is extending $b_1$) and in any case {\sf consumeToken}$()$ returns the content of $K[1]$, in this case $b_k^{tkn_1}$. It follows that a process that grab a token for a block $h$, let us say $b_k^{tkn_h}$, but it is not allowed to consume it is anyway notified with the valid blocks that saturated the set in $K[h]$.


The formal specification of Oracle $\Theta$  abstract data type can be found in \cite{BTADT2018TR}. 

\begin{figure}
	\begin{tikzpicture}[->, auto]
	\tikzset{stato/.style={draw,circle, node distance=4.9cm}}
	\tikzset{dettaglio/.style={black!70}}
	\tikzset{blocco/.style={
			circle,
			inner sep=1pt,
			thick,
			align=center,
			draw=gray,
		}
	}
	
	\node[stato] (0) at (0,0) {$\xi_0 $};
	
	\node[dettaglio, below of=0] (s0) {$\xi_0 = \{$
		\begin{tikzpicture}[scale=0.5, every node/.style={scale=0.5}]	
		\node[] () at (0,7){};
		\node[]() at (-1,4){
			\begin{tabular}{|c|c|c|c}
			\hline
			$\{\}$&$\{\}$&$\{\}$&$\dots$\\
			\hline
			\end{tabular}
		};
		\node[]() at (-4,4) {$K$};
		%		\node[]() at (-1.2,3.5) {\scriptsize $obj_1$};
		%		\node[]() at (-.5,3.5) {\scriptsize $obj_2$};
		%		\node[]() at (.2,3.5) {\scriptsize $\dots$};
		
		\node[]() at (-1,3){
			\begin{tabular}{|c|c|c|c}
			\hline
			{\scriptsize $tkn$}&$\bot$&$\bot$&$\dots$\\
			\hline
			\end{tabular}
		};
		\node[]() at (-4,2) {$tape_{\alpha_2}$};
		
		\node[]() at (-1,2){
			\begin{tabular}{|c|c|c|c}
			\hline
			$\bot$&$\bot$&{\scriptsize $tkn$}&$\dots$\\
			\hline
			\end{tabular}
		};
		\node[]() at (-4,3) {$tape_{\alpha_1}$};
		\node[]() at (-4,1.5) {$\vdots$};	
		\end{tikzpicture}
		$, k\}$};
	
	
	\node[stato, right of=0] (1) {$\xi_1$}; 
	\node[dettaglio, below of=1] (s1) {$\xi_1= \{$			
		\begin{tikzpicture}[scale=0.5, every node/.style={scale=0.5}]	
		\node[] () at (0,7){};
		\node[]() at (-1,4){
			\begin{tabular}{|c|c|c|c}
			\hline
			$\{\}$&$\{\}$&$\{\}$&$\dots$\\
			\hline
			\end{tabular}
		};
		\node[]() at (-4,4) {$K$};
		%		\node[]() at (-1.2,3.5) {\scriptsize $obj_1$};
		%		\node[]() at (-.5,3.5) {\scriptsize $obj_2$};
		%		\node[]() at (.2,3.5) {\scriptsize $\dots$};
		
		\node[]() at (-1,3){
			\begin{tabular}{|c|c|c|c}
			\hline
			{$\bot$}&$\bot$&$\bot$&$\dots$\\
			\hline
			\end{tabular}
		};
		\node[]() at (-4,2) {$tape_{\alpha_2}$};
		
		\node[]() at (-1,2){
			\begin{tabular}{|c|c|c|c}
			\hline
			$\bot$&$\bot$&{\scriptsize $tkn$}&$\dots$\\
			\hline
			\end{tabular}
		};
		\node[]() at (-4,3) {$tape_{\alpha_1}$};
		\node[]() at (-4,1.5) {$\vdots$};	
		\end{tikzpicture}
		$,k\}$};
	
	\path (0) edge [bend left] node[align=center] {\scriptsize {\sf getToken}$(b_1, b_k)/ {b_k^{tkn_1}}$ \\ {\scriptsize{\bf if }$ pop(tape_{\alpha_1})={tkn}$} } (1);
	
	%	\path (0) edge [bend right] node[align=center, below] {\scriptsize {\sf getToken}$(obj_i, obj_k)/ {\sf false}$ \\ {\scriptsize{\bf if } $K[obj_i]=0 \vee pop(m(\alpha_i)={\bot}$} } (1);	
	
	\node[stato, right of=1] (2) {$\xi_2$}; 
	\node[dettaglio, below of=2] (21) {$\xi_2= \{$
		\begin{tikzpicture}[scale=0.5, every node/.style={scale=0.5}]	
		\node[] () at (0,7){};
		\node[]() at (-1.2,4){
			\begin{tabular}{|c|c|c|c}
			\hline
			$\{b_k^{tkn_1}\}$&$\{\}$&$\{\}$&$\dots$\\
			\hline
			\end{tabular}
		};
		\node[]() at (-4,4) {$K$};
		%		\node[]() at (-1.2,3.5) {\scriptsize $obj_1$};
		%		\node[]() at (-.1,3.5) {\scriptsize $obj_2$};
		%		\node[]() at (.5,3.5) {\scriptsize $\dots$};
		
		\node[]() at (-1.6,3){
			\begin{tabular}{|c|c|c|c}
			\hline
			{$\bot$}&$\bot$&$\bot$&$\dots$\\
			\hline
			\end{tabular}
		};
		\node[]() at (-4,2) {$tape_{\alpha_2}$};
		
		\node[]() at (-1.5,2){
			\begin{tabular}{|c|c|c|c}
			\hline
			$\bot$&$\bot$&{\scriptsize $tkn$}&$\dots$\\
			\hline
			\end{tabular}
		};
		\node[]() at (-4,3) {$tape_{\alpha_1}$};
		\node[]() at (-4,1.5) {$\vdots$};	
		\end{tikzpicture}
		$,k \}$};	
	
	\path (1) edge [bend left] node[align=center] {\scriptsize {\sf consumeToken}$({b_k^{tkn_1}})/ \{b_k^{tkn_1}\}$ \\ \scriptsize {\bf if} $|K[1]|<k \wedge {tkn_1} \in \mathfrak{T}$} (2);
\end{tikzpicture}
\caption{A possible path of the transition system defined  by the $\Theta_F$ and  $\Theta_P$-ADTs. We use the following syntax on the edges: {\sf operation}/{\sf output}.}\label{fig:Theta-ADT}
\end{figure}


%%%%%%%%%%%%%%%%%% ORACLE DEF
\begin{comment}
	
We  first introduce some definitions and notations.
\begin{itemize}
	\item $\mathfrak{T}=\{tkn_1,tkn_2, \dots\}$  infinite set of tokens;
	\item $\mathcal{A}=\{\alpha_1, \alpha_2, \dots\}$ an infinite set of rational values;
	\item $\mathcal{M}$ is a countable not empty set of mapping functions $ m(\alpha_i)$ that generate an infinite pseudo random tape $tape_{\alpha_i}$ such that the probability to have in a cell the string $tkn$ is related to a specific $\alpha_i$, $m \in \mathcal{M}: \mathcal{A} \rightarrow \{tkn ,\bot\}^*$; %this function associates to an object a tuple formed by the object and a set of tokens.
	\item ${K}[\ ]$ is a infinite array of sets (one per object) of elements in $\mathcal{B'}$. All the sets are initialized as empty and can be fulfilled with at most $k$ elements, where $k\in \mathbb{N}$ is a parameter of the oracle ADT;
	\item ${pop}: \{tkn ,\bot\}^* \rightarrow \{tkn ,\bot\}^*$, ${pop}(a\cdot w)=w$;
	\item ${head}: \{tkn ,\bot\}^* \rightarrow \{tkn ,\bot\}^*$, ${head}(a\cdot w)=a$;	
	
	\item $add : \{K\} \times \mathbb{N} \times \mathcal{O'} \rightarrow \{K\}$, $add(K, i, obj_{\ell}^{tkn_{h}} )=K$ : $K[i]=K[i] \cup \{obj_{\ell}^{tkn_{h}}\}$ {\bf if} $|K[i]|<k$; {\bf else} $K[i]=K[i]$;
	\item $get : \{K\} \times  \mathbb{N} \rightarrow \mathbb{N}$, $get(K, i)=K[i]$;   
\end{itemize}
%The $\Theta_P$ has the same definition except for the absence of the $K$ array and the $dec$ and $get$ functions.

\definition{\textbf{($\Theta_F$-ADT Definition)}.}\label{def:btadt}
The $\Theta_F$ Abstract Data type is the $6$-tuple 
$\Theta_F$-ADT =$\langle$ A= \{{\sf getToken}$(obj_h,obj_\ell)$, {\sf consumeToken}$( obj_{\ell}^{tkn_{h}}):
obj_h, obj_{\ell}^{tkn_{h}} \in \mathcal{B'}, obj_\ell \in \mathcal{B}, tkn_h \in \mathfrak{T}\}$, B= $\mathcal{B'}  \cup Boolean$, Z= $m(\mathcal{A})^* \times \{K\} \times k \cup \{pop, head, dec, get\}$, $\xi_0, \tau, \delta \rangle$, where the transition function  $\tau:Z \times A \rightarrow Z$ is defined by 
\begin{itemize}
	\item  $\tau( (\{tape_{\alpha_1},\dots, tape_{\alpha_i}, \dots\}, K, k) ,{\sf getToken}(obj_h,obj_\ell))=(\{tape_{\alpha_1},\dots, pop(tape_{\alpha_i}), \dots\}, K, k)$ with $\alpha_i$ the merit of the invoking process;
	\item  $\tau( (\{tape_{\alpha_1},\dots, tape_{\alpha_i}, \dots\}, K, k), {\sf consumeToken}(obj_{\ell}^{tkn_{h}}))= (\{tape_{\alpha_1},\dots, tape_{\alpha_i}, \dots\},$ $ {add}(K, h,obj_{\ell}^{tkn_{h}}))$, if
	$tkn_{h}\in \mathfrak{T}$  ;  $\{ (\{tape_{\alpha_1},\dots, tape_{\alpha_i}, \dots\}, K, k)\}$ otherwise.
	% if $C_{obj}$ is true,
\end{itemize}
and the output function $\delta:Z \times A \rightarrow B$ is defined by 
\begin{itemize}
	\item  $\delta((\{tape_{\alpha_1},\dots, tape_{\alpha_i}, \dots\}, K,k) ,{\sf getToken}(obj_h,obj_\ell))= obj_{\ell}^{tkn_{h}}:  obj_{\ell}^{tkn_{h}} \in \mathcal{O'},tkn_h \in \mathfrak{T}$, if $head(tape_{\alpha_i})=tkn$ with $\alpha_i$ the merit of the invoking process;  $\bot$ otherwise;
	\item  $\delta( (\{tape_{\alpha_1},\dots, tape_{\alpha_i}, \dots\}, K,k) , {\sf consumeToken}(obj_{\ell}^{tkn_{h}}))= {get}(K, h)$.
	
\end{itemize}
%\AD{We assume that we first run the dec and then the get, concerning the consumption.}


\definition{\textbf{($\Theta_P$-ADT Definition)}.}
The $\Theta_P$ Abstract Data type is defined as the $\Theta_F$-ADT with $k=\infty$.

%%%%%%%%%%%%%%%%%% END ORACLE DEF
contenuto...
\end{comment}


\subsection{BT-ADT augmented with $\Theta$ Oracles}
\label{sec:bt-adt-augmented}
In this section we define a specification of the combination of the BT-ADT  with $\Theta$ oracles.
Specifically, we define a refinement of the {\sf append}$(b_\ell)$ operation of the BT-ADT with the oracle operations. %We are considering a refinement (cf. Figure~\ref{fig:Composition}) of the BT-ADT 
When {\sf append}$(b_\ell)$ is invoked then the {\sf getToken}($b_k\leftarrow$last\_block$(f(bt)), b_\ell$) operation is triggered as long as it does not return a token on $b_k$, i.e., ${b_\ell}^{tkn_h}$ which is a valid block in $\mathcal{B'}$. Once obtained, the token is consumed and the append operation terminates, i.e. the block ${b_\ell}^{tkn_h}$ is appended to the blockchain $f(bt)$. Notice that those two operations and the concatenation occur atomically. Figure~\ref{fig:Composition} depicts a possible path of the transition system defined by the refinement. \\ 
We say that the $BT$-$ADT$ augmented with $\Theta_F$ (resp.  $\Theta_P$)  oracle is a \textit{refinement}  $\mathfrak{R}(BT$-$ADT, \Theta_F)$ (resp. $\mathfrak{R}(BT$-$ADT, \Theta_P)$). %The refinment of the {\sf append()} operation is depicted in Figure~\ref{fig:paper-Composition}. 
For space reasons, we invite the reader to read \cite{BTADT2018TR} for their formal specifications.

%%%%% COMPOSIZIONE
\begin{figure}
	\centering
	\begin{tikzpicture}[->, auto]
	\tikzset{stato/.style={draw,circle, node distance=4.4cm}}
	\tikzset{dettaglio/.style={black!70},node/.style={scale=0.6}}
	\tikzset{blocco/.style={
			circle,
			inner sep=1pt,
			thick,
			align=center,
			draw=gray,
		}
	}	
	%miniatura
	\node[] () at (5,4) {
		\begin{tikzpicture}[->, auto, scale=0.5, every node/.style={scale=0.8}]
		
		
		\node[stato] (0) at (0,0) {$\xi_0 $};
		
		\node[dettaglio, below of=0] (s0) {$\xi_0 = \{$
			\begin{tikzpicture}[scale=0.8, every node/.style={scale=0.8}]	
			\node  [blocco] (i11) at (0.5,3)  {\scriptsize $b_0$};	
			\end{tikzpicture}
			$,f,P\}$};
		
		
		\node[stato, right of=0] (1) {$\xi_1$}; 
		\node[dettaglio, below of=1] (s1) {$\xi_1= \{$			
			\begin{tikzpicture}[scale=0.8, every node/.style={scale=0.8}]	
			\node  [blocco] (i11) at (0.5,3)  {\scriptsize $b_0$};
			\node  [blocco]  (i12) at (1.2,3) {\scriptsize $b_k$};
			\draw[<-] (i11) edge (i12)  ;
			\end{tikzpicture}
			$ ,f,P \}$};
		
		\path (0) edge [bend left] node[align=center] {\scriptsize {\sf append}$( b_k)/ {\sf true}$ \\ {\scriptsize{\bf if } $b_k \in \mathcal{B'} $}} (1);
		\path (0) edge [loop left] node[align=center] {\scriptsize {\sf append}$(b_3)/ {\sf false}$ \\ {\scriptsize{\bf if } $b_3 \notin \mathcal{B'} $}} (0);	
		
		
		\node[stato, right of=1] (2) {$\xi_2$}; 
		\node[dettaglio, below of=2] (21) {$\xi_2= \{$
			\begin{tikzpicture}[scale=0.8, every node/.style={scale=0.8}]
			\node  [blocco] (i11) at (0.5,3)  {\scriptsize $b_0$};
			\node  [blocco]  (i12) at (1.3,3.2) {\scriptsize $b_k$};
			\node [blocco] (i13) at (1.3,2.7) {\scriptsize $b_2$};
			\draw[<-] (i11) edge (i12) (i11) edge (i13) ;
			\end{tikzpicture}
			$ f,P \}$};	
		
		\path (1) edge [bend left] node[align=center] {\scriptsize {\sf append}$( b_2)/ {\sf true}$ \\ {\scriptsize{\bf if } $b_2 \in \mathcal{B'} $}} (2);
		\path (1) edge [loop right] node[align=center] {\scriptsize {\sf append}$(b_4)/ {\bot}$ \\ {\scriptsize{\bf if } $b_4 \notin \mathcal{B'} $}} (1);
		
		
		\path (1) edge [loop above] node[align=center] {\scriptsize {\sf read}$()/ {b_0 \frown b_k}$} (1);	
		\path (2) edge [loop above] node[align=center] {\scriptsize {\sf read}$()/ {b_0 \frown b_2}$} (2);	
		
		\draw[thick] (-.4,-1.3) rectangle (9,3);	
	\end{tikzpicture}
};%fine figura in miniatura



\node[stato] (0) at (0,0) {$\xi_0^\prime $};

\node[dettaglio, below of=0] (s0) {$\{$
	\begin{tikzpicture}[scale=0.5, every node/.style={scale=0.5}]	
	\node[] () at (0,7){};
	\node[]() at (-.9,4){
		\begin{tabular}{|c|c|c}
		\hline
		$\{\}$&$\{\}$&$\dots$\\
		\hline
		\end{tabular}
	};
	\node[]() at (-3,4) {$K$};
	%	\node[]() at (-1.2,3.5) {\scriptsize $obj_1$};
	%	\node[]() at (-.5,3.5) {\scriptsize $obj_2$};
	%	\node[]() at (.2,3.5) {\scriptsize $\dots$};
	
	\node[]() at (-.9,3){
		\begin{tabular}{|c|c|c}
		\hline
		{\scriptsize $tkn$}&$\bot$&$\dots$\\
		\hline
		\end{tabular}
	};
	\node[]() at (-3,2) {$tape_{\alpha_2}$};
	
	\node[]() at (-.9,2){
		\begin{tabular}{|c|c|c}
		\hline
		$\bot$&{\scriptsize $tkn$}&$\dots$\\
		\hline
		\end{tabular}
	};
	\node[]() at (-3,3) {$tape_{\alpha_1}$};
	\node[]() at (-3,1.5) {$\vdots$};	
	\end{tikzpicture},$k$,
	\begin{tikzpicture}[scale=0.8, every node/.style={scale=0.8}]
	\node  [blocco] (i11) at (0.5,3)  {\scriptsize $b_0$};
	\end{tikzpicture}
	$,f,P\}$};

%, right of=0
\node[stato] (1) at (5.2,0) {$\xi_{1/a}^\prime$}; 
\node[dettaglio, below of=1] (s1) {$ \{$			
	\begin{tikzpicture}[scale=0.5, every node/.style={scale=0.5}]	
	\node[] () at (-2,7){};
	\node[]() at (-2.5,4){
		\begin{tabular}{|c|c|c}
		\hline
		$\{\}$&$\{\}$&$\dots$\\
		\hline
		\end{tabular}
	};
	%	\node[]() at (-3,4) {$K$};
	%	\node[]() at (-1.2,3.5) {\scriptsize $obj_1$};
	%	\node[]() at (-.5,3.5) {\scriptsize $obj_2$};
	%	\node[]() at (.2,3.5) {\scriptsize $\dots$};
	
	\node[]() at (-2.5,3){
		\begin{tabular}{|c|c|c}
		\hline
		{$\bot$}&$\bot$&$\dots$\\
		\hline
		\end{tabular}
	};
	%\node[]() at (-3,2) {$tape_{\alpha_2}$};
	
	\node[]() at (-2.5,2){
		\begin{tabular}{|c|c|c}
		\hline
		$\bot$&{\scriptsize $tkn$}&$\dots$\\
		\hline
		\end{tabular}
	};
	%\node[]() at (-3,3) {$tape_{\alpha_1}$};
	\node[]() at (-3,1.5) {$\vdots$};	
	\end{tikzpicture},$k$,
	\begin{tikzpicture}[scale=0.8, every node/.style={scale=0.8}]
	\node  [blocco] (i11) at (0.5,3)  {\scriptsize $b_0$};
	\end{tikzpicture}
	$,f,P\}$};
\path (0) edge [bend left] node[align=center] {\scriptsize {\sf getToken}$(b_1\leftarrow$last\_block$(f(bt)), b_k)/{b_k^{tkn_1}}$ \\ {\scriptsize{\bf if } $pop(tape_{\alpha_1})={tkn}$} } (1);

%	\path (0) edge [bend right] node[align=center, below] {\scriptsize {\sf getToken}$(obj_i, obj_k)/ {\sf false}$ \\ {\scriptsize{\bf if } $K[obj_i]=0 \vee pop(m(\alpha_i)={\bot}$} } (1);	

\node[stato, right of=1] (2) {$\xi_{1/b}^\prime$}; 
\node[dettaglio, below of=2] (21) {$ \{$
	\begin{tikzpicture}[scale=0.5, every node/.style={scale=0.5}]	
	\node[] () at (-4,7){};
	\node[]() at (-2.5,4){
		\begin{tabular}{|c|c|c}
		\hline
		$\{b_k^{tkn_1}\}$&$\{\}$&$\dots$\\
		\hline
		\end{tabular}
	};
	%	\node[]() at (-3,4) {$K$};
	%	\node[]() at (-1.2,3.5) {\scriptsize $obj_1$};
	%	\node[]() at (-.1,3.5) {\scriptsize $obj_2$};
	%	\node[]() at (.5,3.5) {\scriptsize $\dots$};
	
	\node[]() at (-3,3){
		\begin{tabular}{|c|c|c}
		\hline
		{$\bot$}&$\bot$&$\dots$\\
		\hline
		\end{tabular}
	};
	%	\node[]() at (-3,2) {$tape_{\alpha_2}$};
	
	\node[]() at (-2.9,2){
		\begin{tabular}{|c|c|c}
		\hline
		$\bot$&{\scriptsize $tkn$}&$\dots$\\
		\hline
		\end{tabular}
	};
	%\node[]() at (-3,3) {$tape_{\alpha_1}$};
	\node[]() at (-3,1.5) {$\vdots$};	
	\end{tikzpicture},$k$,
	\begin{tikzpicture}[scale=0.8, every node/.style={scale=0.8}]
	\node  [blocco] (i11) at (0.5,3)  {\scriptsize $b_0$};
	\node  [blocco]  (i12) at (1.3,3) {\scriptsize $b_1$};
	\draw[<-] (i11) edge (i12)  ;
	\end{tikzpicture}
	$,f,P \}$};	

\path (1) edge [bend left] node[align=center] {\scriptsize {\sf consumeToken}$(b_k^{tkn_1})/\{b_k^{tkn_1}\}$ \\ {\scriptsize {\bf if} $|K[1]|<k \wedge b_k^{tkn_1} \in \mathfrak{T}$}  }  (2);

\draw[thick] (-2.1,-2.7) rectangle (11.9,2.5); 
\draw[-, dotted] (2,3.2)-- (-2.1,2.5);
\draw[-, dotted] (12,2.5)-- (6,3.2);
\end{tikzpicture}


\caption{A possible path of the transition system  defined by the refinement of the {\sf append}$()$ operation. We use the following syntax on the edges: {\sf operation}/{\sf output}.}\label{fig:Composition}
\end{figure}
  

%\begin{figure*}[t]
%	\centering
%	\fbox{
%		\begin{minipage}{0.4\textwidth}
%			%\footnotesize
%			\scriptsize
%			%\renewcommand{\baselinestretch}{2.5}
%			\begin{tabbing}
%				aaaA\=aA\=aA\=aaaA\kill
%				
%				{\bf Init}:\\
%				
%				\line{} \> $token \leftarrow \bot;$\\
%				\line{} \> $bt_i \leftarrow b_0;$\\
%				\line{} \> $\dots$\\
%				
%				%				~---------------------------------------------------------------------\\
%				%				
%				%				{\bf upon} ${\sf append}(b_\ell)$:\\
%				%				\line{} \> $\dots$\\
%				%				\line{} \> {\bf while} ${\sf true}$; \\
%				%				\line{} \>\>$token \leftarrow \sf{getToken}(b_h \leftarrow\textnormal{last\_block}(f(bt)),b_\ell)$;\\
%				%				\line{} \>\>{\bf if} $token \neq \bot$ {\bf then break};\\
%				%				%\line{}\>\> $\dots$\\
%				%				%\line{} \> $\dots$\\
%				%				\line{} \> {\sf consumeToken}$(token) \wedge \{b_0\}^\frown {f(bt)}^ \frown \{b\}$;\\
%				%				\line{} \>$token \leftarrow \bot$;\\
%				%				\line{}\>$\dots$\\
%				
%			\end{tabbing}
%			\normalsize
%		\end{minipage}%
%		\hspace{1.5cm}
%		\begin{minipage}{0.4\textwidth}
%			%\footnotesize
%			\scriptsize
%			%\renewcommand{\baselinestretch}{2.5}
%			\begin{tabbing}
%				aaaA\=aA\=aA\=aaaA\kill
%				
%				%			{\bf Init}\\
%				%			
%				%			\line{} \> $token \leftarrow \bot;$\\
%				%			\line{} \> $bt_i \leftarrow b_0;$\\
%				%			\line{} \> $\dots$\\
%				%			
%				%			~---------------------------------------------------------------------\\
%				
%				{\bf upon} ${\sf append}(b_\ell)$:\\
%				\line{} \> $\dots$\\
%				\line{} \> {\bf while} $(token = \bot)$: \\
%				\line{} \>\>$token \leftarrow \sf{getToken}(b_h \leftarrow\textnormal{last\_block}(f(bt)),b_\ell)$;\\
%				%\line{} \>\>{\bf if} $token \neq \bot$ {\bf then break};\\
%				%\line{}\>\> $\dots$\\
%				%\line{} \> $\dots$\\
%				\line{} \> {\sf consumeToken}$(token) \wedge \{b_0\}^\frown {f(bt)}^ \frown \{b\}$;\\
%				\line{} \>$token \leftarrow \bot$;\\
%				\line{}\>$\dots$\\
%				
%			\end{tabbing}
%			\normalsize
%		\end{minipage}
%	}
%	\caption{A generic implementation fragment of the $\mathfrak{R}(BT$-$ADT, \Theta)$ for the {\sf append}$()$ operation . }
%	\label{fig:generic-ImplementationM}   
%\end{figure*}
The following theorem state that the obtained refinement enjoys the\textit{ $k$-fork coherence,} i.e. no more than $k$ forks may happen, respectively. For space reasons the proof can be found in \cite{BTADT2018TR}.
%\vspace{0.1cm}
%\begin{theorem}[{Append termination}]\label{t:appendTerminationM}
%	Let $H=\langle \Sigma, E, \Lambda, \mapsto, \prec, \nearrow \rangle$ be any concurrent history generated by $\mathfrak{R}(BT$-$ADT, \Theta_P)$. Then %verifies the Append termination, i.e. 
%	each invoked {\sf append}$()$ operation in $H$ eventually successfully terminates. 
%\end{theorem}

% \begin{proofT}
% 	We prove the theorem by considering the defined refinement (cf. Figure \ref{fig:genericImplementation})  where \emph{(i)} there are  a infinite number of ${\sf getToken}()$ invocations for  object $obj$ and \emph{(ii)} given a valid block as input parameter, the {\sf consumeToken}$()$ operation always successfully terminates by definition of Oracle 
% $\Theta_P$ (as $k$ is infinite). From  the properties of the pseudo random sequences of tapes, if there are an infinite number of ${\sf getToken}()$ invocations for  object $obj$ then there exists at least one response for which ${\sf getToken}()$ operation returns a valid block, thus when passed as input of the {\sf consumeToken}$()$ operation,  such operation successfully terminates. 
% 	\renewcommand{\toto}{t:appendTermination}
% \end{proofT} 

\begin{definition}[$k$-Fork coherence]
	A concurrent history $H=\langle \Sigma, E, \Lambda, \mapsto, \prec, \nearrow \rangle$ of  $\mathfrak{R}(BT$-$ADT, \Theta_P)$ satisfies the \emph{k-Fork coherence} if there are at most $k$ {\sf append}$()$ operations that return $\top$ for the same token. 
\end{definition}


\begin{theorem}[k-Fork coherence]\label{t:kForkM}
	Any concurrent history $H=\langle \Sigma, E, \Lambda, \mapsto, \prec, \nearrow \rangle$ of the  $\mathfrak{R}(BT$-$ADT, \Theta_F)$ satisfies the \emph{k-Fork Coherence}.
\end{theorem}

% \begin{proofT}
% 	We prove the theorem by considering the defined refinement (cf. Figure \ref{fig:genericImplementation}) where  \emph{(i)} there are a infinite number of ${\sf getToken}()$ invocations for object $obj$ and \emph{(ii)} given a valid block as input parameter, the {\sf consumeToken}$()$ operation successfully terminates if it has been invoked less than $k$ times for the same token. 
% 	From the properties of the pseudo random sequences of tapes, if there are an infinite number of ${\sf getToken}()$ invocations for object $obj$ then there exists at least one response for which ${\sf getToken}()$ operation returns a token $t$, which, when passed as input of the {\sf consumeToken}$()$ operation it successfully terminates if at most $k-1$ tokens $t$ have been already consumed. 	
% 	\renewcommand{\toto}{t:kFork}
% \end{proofT} 



%%%%% COMPOSIZIONE
%\begin{figure}
%	\centering
%	\begin{tikzpicture}[->, auto]
%	\tikzset{stato/.style={draw,circle, node distance=5.7cm}}
%	\tikzset{dettaglio/.style={black!70}}
%	\tikzset{blocco/.style={
%			circle,
%			inner sep=1pt,
%			thick,
%			align=center,
%			draw=gray,
%		}
%	}	
%	%miniatura
%	\node[] () at (5,4) {
%		\begin{tikzpicture}[->, auto, scale=0.5, every node/.style={scale=0.5}]
%		
%		
%		\node[stato] (0) at (0,0) {$\xi_0 $};
%		
%		\node[dettaglio, below of=0] (s0) {$\xi_0 = \{$
%			\begin{tikzpicture}[scale=0.8, every node/.style={scale=0.8}]	
%			\node  [blocco] (i11) at (0.5,3)  {\scriptsize $b_0$};	
%			\end{tikzpicture}
%			$f\}$};
%		
%		
%		\node[stato, right of=0] (1) {$\xi_1$}; 
%		\node[dettaglio, below of=1] (s1) {$\xi_1= \{$			
%			\begin{tikzpicture}[scale=0.8, every node/.style={scale=0.8}]	
%			\node  [blocco] (i11) at (0.5,3)  {\scriptsize $b_0$};
%			\node  [blocco]  (i12) at (1.2,3) {\scriptsize $b_k$};
%			\draw[<-] (i11) edge (i12)  ;
%			\end{tikzpicture}
%			$ f \}$};
%		
%		\path (0) edge [bend left] node[align=center] {\scriptsize {\sf append}$( b_k)/ {\sf true}$ \\ {\scriptsize{\bf if } $b_k \in \mathcal{B'} $}} (1);
%		\path (0) edge [loop left] node[align=center] {\scriptsize {\sf append}$(b_3)/ {\sf false}$ \\ {\scriptsize{\bf if } $b_3 \notin \mathcal{B'} $}} (0);	
%		
%		
%		\node[stato, right of=1] (2) {$\xi_2$}; 
%		\node[dettaglio, below of=2] (21) {$\xi_2= \{$
%			\begin{tikzpicture}[scale=0.8, every node/.style={scale=0.8}]
%			\node  [blocco] (i11) at (0.5,3)  {\scriptsize $b_0$};
%			\node  [blocco]  (i12) at (1.3,3.2) {\scriptsize $b_k$};
%			\node [blocco] (i13) at (1.3,2.7) {\scriptsize $b_2$};
%			\draw[<-] (i11) edge (i12) (i11) edge (i13) ;
%			\end{tikzpicture}
%			$ f \}$};	
%		
%		\path (1) edge [bend left] node[align=center] {\scriptsize {\sf append}$( b_2)/ {\top}$ \\ {\scriptsize{\bf if } $b_2 \in \mathcal{B'} $}} (2);
%		\path (1) edge [loop right] node[align=center] {\scriptsize {\sf append}$(b_4)/ {\bot}$ \\ {\scriptsize{\bf if } $b_4 \notin \mathcal{B'} $}} (1);
%		
%		
%		\path (1) edge [loop above] node[align=center] {\scriptsize {\sf read}$()/ {b_0 \frown b_k}$} (1);	
%		\path (2) edge [loop above] node[align=center] {\scriptsize {\sf read}$()/ {b_0 \frown b_2}$} (2);	
%		
%		\draw[thick] (-1.2,-1.3) rectangle (7,2);	
%	\end{tikzpicture}
%};%fine figura in miniatura
%
%
%
%\node[stato] (0) at (0,0) {$\xi_0^\prime $};
%
%\node[dettaglio, below of=0] (s0) {$\xi_0^\prime = \{$
%	\begin{tikzpicture}[scale=0.5, every node/.style={scale=0.5}]	
%	\node[] () at (0,7){};
%	\node[]() at (-.8,4){
%		\begin{tabular}{|c|c|c|c}
%		\hline
%		$k$&$k$&$k$&$\dots$\\
%		\hline
%		\end{tabular}
%	};
%	\node[]() at (-3,4) {$K$};
%	\node[]() at (-1.2,3.5) {\scriptsize $obj_1$};
%	\node[]() at (-.5,3.5) {\scriptsize $obj_2$};
%	\node[]() at (.2,3.5) {\scriptsize $\dots$};
%	
%	\node[]() at (-.6,3){
%		\begin{tabular}{|c|c|c|c}
%		\hline
%		{\scriptsize $tkn$}&$\bot$&$\bot$&$\dots$\\
%		\hline
%		\end{tabular}
%	};
%	\node[]() at (-3,2) {$tape_{\alpha_2}$};
%	
%	\node[]() at (-.6,2){
%		\begin{tabular}{|c|c|c|c}
%		\hline
%		$\bot$&$\bot$&{\scriptsize $tkn$}&$\dots$\\
%		\hline
%		\end{tabular}
%	};
%	\node[]() at (-3,3) {$tape_{\alpha_1}$};
%	\node[]() at (-3,1.5) {$\vdots$};	
%	\end{tikzpicture}
%	\begin{tikzpicture}[scale=0.8, every node/.style={scale=0.8}]
%	\node  [blocco] (i11) at (0.5,3)  {\scriptsize $b_0$};
%	\end{tikzpicture}
%	$f\}$};
%
%%, right of=0
%\node[stato] (1) at (5.2,0) {$\xi_{1/a}^\prime$}; 
%\node[dettaglio, below of=1] (s1) {$\xi_{1/a}^\prime= \{$			
%	\begin{tikzpicture}[scale=0.5, every node/.style={scale=0.5}]	
%	\node[] () at (0,7){};
%	\node[]() at (-.8,4){
%		\begin{tabular}{|c|c|c|c}
%		\hline
%		$k$&$k$&$k$&$\dots$\\
%		\hline
%		\end{tabular}
%	};
%	\node[]() at (-3,4) {$K$};
%	\node[]() at (-1.2,3.5) {\scriptsize $obj_1$};
%	\node[]() at (-.5,3.5) {\scriptsize $obj_2$};
%	\node[]() at (.2,3.5) {\scriptsize $\dots$};
%	
%	\node[]() at (-.6,3){
%		\begin{tabular}{|c|c|c|c}
%		\hline
%		{$\bot$}&$\bot$&$\bot$&$\dots$\\
%		\hline
%		\end{tabular}
%	};
%	\node[]() at (-3,2) {$tape_{\alpha_2}$};
%	
%	\node[]() at (-.6,2){
%		\begin{tabular}{|c|c|c|c}
%		\hline
%		$\bot$&$\bot$&{\scriptsize $tkn$}&$\dots$\\
%		\hline
%		\end{tabular}
%	};
%	\node[]() at (-3,3) {$tape_{\alpha_1}$};
%	\node[]() at (-3,1.5) {$\vdots$};	
%	\end{tikzpicture}
%	\begin{tikzpicture}[scale=0.8, every node/.style={scale=0.8}]
%	\node  [blocco] (i11) at (0.5,3)  {\scriptsize $b_0$};
%	\end{tikzpicture}
%	$f\}$};
%\path (0) edge [bend left] node[align=center] {\scriptsize {\sf getToken}$($last\_block$(f(bt))=b_1, b_k)/{b_k^{tkn_1}}$ \\ {\scriptsize{\bf if } $pop(tape_{\alpha_1})={tkn}$} } (1);
%
%%	\path (0) edge [bend right] node[align=center, below] {\scriptsize {\sf getToken}$(obj_i, obj_k)/ {\sf false}$ \\ {\scriptsize{\bf if } $K[obj_i]=0 \vee pop(m(\alpha_i)={\bot}$} } (1);	
%
%\node[stato, right of=1] (2) {$\xi_{1/b}^\prime$}; 
%\node[dettaglio, below of=2] (21) {$\xi_{1/b}^\prime= \{$
%	\begin{tikzpicture}[scale=0.5, every node/.style={scale=0.5}]	
%	\node[] () at (0,7){};
%	\node[]() at (-.8,4){
%		\begin{tabular}{|c|c|c|c}
%		\hline
%		$k-1$&$k$&$k$&$\dots$\\
%		\hline
%		\end{tabular}
%	};
%	\node[]() at (-3,4) {$K$};
%	\node[]() at (-1.2,3.5) {\scriptsize $obj_1$};
%	\node[]() at (-.1,3.5) {\scriptsize $obj_2$};
%	\node[]() at (.5,3.5) {\scriptsize $\dots$};
%	
%	\node[]() at (-.8,3){
%		\begin{tabular}{|c|c|c|c}
%		\hline
%		{$\bot$}&$\bot$&$\bot$&$\dots$\\
%		\hline
%		\end{tabular}
%	};
%	\node[]() at (-3,2) {$tape_{\alpha_2}$};
%	
%	\node[]() at (-.8,2){
%		\begin{tabular}{|c|c|c|c}
%		\hline
%		$\bot$&$\bot$&{\scriptsize $tkn$}&$\dots$\\
%		\hline
%		\end{tabular}
%	};
%	\node[]() at (-3,3) {$tape_{\alpha_1}$};
%	\node[]() at (-3,1.5) {$\vdots$};	
%	\end{tikzpicture}
%	\begin{tikzpicture}[scale=0.8, every node/.style={scale=0.8}]
%	\node  [blocco] (i11) at (0.5,3)  {\scriptsize $b_0$};
%	\node  [blocco]  (i12) at (1.3,3) {\scriptsize $b_1$};
%	\draw[<-] (i11) edge (i12)  ;
%	\end{tikzpicture}
%	$f \}$};	
%
%\path (1) edge [bend left] node[align=center] {\scriptsize {\sf consumeToken}$(b_k^{tkn_1})/\top$ \\ {\scriptsize {\bf if} $K[1]>0 \wedge b_k^{tkn_1} \in \mathfrak{T}$}  }  (2);
%
%\draw[thick] (-2.5,-2.7) rectangle (13.8,2.5); 
%\draw[-, dotted] (2,3.2)-- (-2.5,2.5);
%\draw[-, dotted] (14,2.5)-- (6,3.2);
%\end{tikzpicture}
%
%
%\caption{Refinement of the {\sf append}$()$ operation. On the edges: {\sf operation}/{\sf output}.}\label{fig:paper-Composition}
%\end{figure}


\subsection{Hierarchy}
\label{sec:hierarchy}


We propose a hierarchy between BT-ADTs  augmented with oracle ADTs. We use the following notation:  BT-ADT$_{SC}$ and BT-ADT$_{E C}$ to refer respectively to BT-ADT generating concurrent histories that satisfy the $SC$ and the $E C$ consistency criteria. When augmented with the oracles we have the following four typologies, where for the \emph{frugal} oracle we explicit the value of $k$: $\mathfrak{R}(\text{BT-ADT}_{SC}, \Theta_{F,k})$, $\mathfrak{R}(\text{BT-ADT}_{SC}, \Theta_P)$, $\mathfrak{R}(\text{BT-ADT}_{ E C}, \Theta_{P})$, $\mathfrak{R}(\text{BT-ADT}_{E C}, \Theta_{F,k})$.
We aim at studying the relationship among the different refinements. Without loss of generality, let us consider only the set of histories $\hat{\mathcal{H}}^{\mathfrak{R}(\text{BT-ADT},\Theta)}$ such that each history $\hat{H}^{\mathfrak{R}(\text{BT-ADT},\Theta)} \in \hat{\mathcal{H}}^{\mathfrak{R}(BT,\Theta)}$  is purged of unsuccessful {\sf append}$()$ response events (i.e., such that the returned value is $\bot$). Let $\hat{\mathcal{H}}^{\mathfrak{R}(\text{BT-ADT},\Theta_F)}$ be the concurrent set of histories generated by a BT-ADT enriched with $\Theta_F$-ADT and let $\hat{\mathcal{H}}^{\mathfrak{R}(\text{BT-ADT},\Theta_P)}$ be the concurrent set of histories generated by a BT-ADT enriched with $\Theta_P$-ADT. All the theorems are proven in \cite{BTADT2018TR}.

\begin{theorem}\label{t:oracolsHierarchyM}
	$\hat{\mathcal{H}}^{\mathfrak{R}(\text{BT-ADT},\Theta_F)} \subseteq \hat{\mathcal{H}}^{\mathfrak{R}(\text{BT-ADT},\Theta_P)}$. 
\end{theorem}

\begin{theorem}\label{t:oracolsHierarchyFM}
	If $k_1 \leq k_2$ then $\hat{\mathcal{H}}^{\mathfrak{R}(\text{BT-ADT},\Theta_{F,k_1})} \subseteq \hat{\mathcal{H}}^{\mathfrak{R}(\text{BT-ADT},\Theta_{F,k_2})}$. 
\end{theorem}

Finally, from Theorem \ref{th:strongImpliesEventualM} the next corollary follows.

\begin{corollary}\label{c:oracolsHierarchySameOracleM}
	$\hat{\mathcal{H}}^{(\mathfrak{R}(\text{BT-ADT}_{SC},\Theta)} \subseteq \hat{\mathcal{H}}^{\mathfrak{R}(\text{BT-ADT}_{E C},\Theta)}$. 
\end{corollary}

The above results imply the hierarchy depicted in Figure \ref{fig:BTHierarchyPurgedM}.

\begin{figure}
	\centering
	\begin{tikzpicture}[scale=0.9]
	
	\node[draw](1) at (0,2) {$\mathfrak{R}(\text{BT-ADT}_{SC}, \Theta_{F,k=1})$};
	\node[draw](2) at (-2,-2) {$\mathfrak{R}(\text{BT-ADT}_{ E C}, \Theta_{F,k>1})$};
	
	\node[draw, gray!40](3) at (2.5,-1) {$\mathfrak{R}(\text{BT-ADT}_{ SC}, \Theta_{P})$};
	\node[draw,  gray!40](5) at (-2,0) { $\mathfrak{R}(\text{BT-ADT}_{ SC}, \Theta_{F,k>1})$};
	\node[draw](4) at (0,-4) {$\mathfrak{R}(\text{BT-ADT}_{ E C}, \Theta_{P})$};
	
	%	\draw[->, gray!30]
	%	;
	
	\draw[->]  (2) edge (4) (5) edge (2) 	(1) edge (3)
	(1) edge (5)	(3) edge (4) ;
	
	%\draw[->] (-5.2,1)--(-5.2,-5); \node[rotate=90] () at (-5.5,-3) {Weaker BT properties};
	
	\node[] () at (-2, 1.3) {\scriptsize Theorem \ref{t:oracolsHierarchyFM}};
	\node[] () at (-2.5, 0.7) {\scriptsize Theorem \ref{t:noForkBeStrong}};
	\node[] () at (2.5, 1) {\scriptsize Theorem \ref{t:oracolsHierarchyM}};
	\node[] () at (3, 0) {\scriptsize Theorem \ref{t:noForkBeStrong}};	
	\node[] () at (-2.2, -3) {\scriptsize Theorem \ref{t:oracolsHierarchyM}};
	\node[] () at (-3.2, -1) {\scriptsize Corollary \ref{c:oracolsHierarchySameOracleM}};
	\node[] () at (3, -2.5) {\scriptsize Corollary \ref{c:oracolsHierarchySameOracleM}};			
	\end{tikzpicture}
	\caption{$\mathfrak{R}(\text{BT-ADT}, \Theta)$ Hierarchy. In gray we anticipate the combinations impossible in a message-passing system due to Theorem \ref{t:noForkBeStrong}.}\label{fig:BTHierarchyPurgedM}
\end{figure}


\section{Implementing BT-ADTs}
\label{sec:comm-abstr-bt}
An interested reader can find all the proofs of Lemmas and Theorems of this section in \cite{BTADT2018TR}.

\subsection{Implementability in a concurrent model}
In this Section we show that $\Theta_{F,k=1}$ has consensus number $\infty$ and that $\Theta_{P}$ %with k unbounded 
has consensus number 1.
We consider a concurrent system composed by $n$ processes such that up to $f$ processes are faulty (stop prematurely by crashing), $f<n$. Moreover, processes can communicate through atomic registers.

\subsubsection{Frugal with $k=1$ at least as strong as Consensus}
In the following we prove that there exists a wait-free implementation of the Consensus \cite{lamport1982byzantine} by the $\Theta_{F,k=1}$ Oracle object. In particular, we consider a version of the Consensus problem for the blockchain. Thus, we consider the Validity property as in \cite{redbelly17} such that the decided block $b$ satisfies the predicate $P$. 
\begin{definition}
	Consensus $\mathcal{C}$:
	\begin{itemize}
		\item \textbf{Termination.} Every correct process eventually decides some value.
		\item \textbf{Integrity.} No correct process decides twice.
		\item \textbf{Agreement.} If there is a correct process that decides a value $b$, then eventually all the correct processes decide $b$.
		\item \textbf{Validity\cite{redbelly17}.} A decided value is valid, it satisfies the predefined predicate denoted $P$.
	\end{itemize}
\end{definition}


%Formally, $\mathcal{C}$ reduces to $\Theta_{F,k=1}$ if there exists a distributed algorithm $\mathcal{T}_{\mathcal{C}\rightarrow \Theta_{F,k=1}}$ which emulates $\mathcal{C}$ when employing  $\Theta_{F,k=1}$.
We first show that there exists a wait-free implementation of {\sf Compare\&Swap}$()$ object by {\sf consumeToken}$()$ object in the case of $\Theta_{F,k=1}$, implying that {\sf consumeToken}$()$ has the same Consensus number as {\sf Compare\&Swap}$()$ which is $\infty$ (see \cite{herlihy1991wait}). Finally we compose the {\sf consumeToken}$()$ with the {\sf getToken}$()$ object proving that there exist a wait-free implementation of $\mathcal{C}$ by $\Theta_{F,k=1}$.

Figure \ref{fig:CAS} describes {\sf consumeToken}$()$ (CT), as specified by the $\Theta$-ADT, along with the {\sf Compare\&Swap}$()$ (CAS). In Figure \ref{fig:CAStoCT} an implementation of CAS by CT. %{\sf Compare\&Swap}$()$ takes three parameters as input, the $register$, the $old\_value$ and the $new\_value$. If the value in $register$ is the same as  $old\_value$ then the $new\_value$ is stored in $register$ and in any case the operation returns the value that was in $register$ at the beginning of the operation. 
%In comparison with {\sf consumeToken}$(b_\ell^{tkn_h})$ we have that $b_\ell^{tkn_h}$ is the $new\_value$, $register$ is $K[h]$ and the implicit $old\_value$ is $\{\}$. That is, $add(K,h,b)$ stores $b$ in $K[h]$ if $|K[h]|<k=1$, then if $K[h]=\{\}$. In any case the operation returns the content of $K[h]$ at the end of the operation itself. Figure \ref{fig:CAStoCT} describes and algorithm that reduces CAS to {\sf consumeToken}$()$.

\begin{figure*}[t]
	\centering
	\fbox{
		\begin{minipage}{0.4\textwidth}
			%\footnotesize
			\scriptsize
			\resetline
			%\renewcommand{\baselinestretch}{2.5}
			\begin{tabbing}
				aaaA\=aA\=aA\=aaaA\kill
				\line{} {\sf consumeToken}$(b_\ell^{tkn_h}):$\\
				\line{} \> $previous\_value \leftarrow K[h];$\\
				\line{} \> {\bf if} $(previous\_value == \{\} \wedge tkn_h \in \mathfrak{T})${\bf then};\\
				\line{} \>\>$K[h] \leftarrow K[h] \cup \{b_\ell^{tkn_h}\}$;\\
				\line{} \>\> {\bf endIf}\\
				\line{} \> {\bf return} $K[h]$\\
			\end{tabbing}
			\normalsize
		\end{minipage}%
		\vspace{.5cm}
		\begin{minipage}{0.4\textwidth}
			%\footnotesize
			\scriptsize
			\resetline
			%\renewcommand{\baselinestretch}{2.5}
			\begin{tabbing}
				aaaA\=aA\=aA\=aaaA\kill
				\line{} {\sf compare\&swap}$(register, old\_value, new\_value):$\\
				\line{} \> $previous\_value \leftarrow register;$\\
				\line{} \> {\bf if} $(previous\_value == old\_value)${\bf then};\\
				\line{} \>\>$register \leftarrow new\_value$;\\
				\line{} \>\> {\bf endIf}\\
				\line{} \> {\bf return} $previous\_value$\\
			\end{tabbing}
			\normalsize
		\end{minipage}
		
	}
	\caption{{\sf Compare\&Swap}$()$ and {\sf consumeToken}$()$ in the case of $\Theta_{F,k=1}$.}
	\label{fig:CAS}   
\end{figure*}

\begin{figure*}[t]
	\centering
	\fbox{
		\begin{minipage}{0.4\textwidth}
			%\footnotesize
			\scriptsize
			\resetline
			%\renewcommand{\baselinestretch}{2.5}
			\begin{tabbing}
				aaaA\=aA\=aA\=aaaA\kill
				\line{} {\sf compare\&swap}$(K[h], \{\}, b_\ell^{tkn_h}):$\\
				\line{}\> $returned\_value\leftarrow${\sf consumeToken}$(b_\ell^{tkn_h});$\\
				\line{CAStoCT-03} \> {\bf if} $(returned\_value == b_\ell^{tkn_h})${\bf then};\\
				\line{} \>\>{\bf return} $\{\}$;\\
				\line{} \>\> {\bf else} {\bf return} $returned\_value$;\\
				\line{} \>\> {\bf endIf} \\
			\end{tabbing}
			\normalsize
		\end{minipage}	
	}
	\caption{An implementation of CAS by {\sf consumeToken}$()$ in the case of $\Theta_{F,k=1}$.}
	\label{fig:CAStoCT}   
\end{figure*}


\begin{theorem}\label{t:CAStoCT}
	If input values are in $\mathcal{B'}$ then there exists an implementation of CAS by CT in the case of $\Theta_{F,k=1}$.
\end{theorem}

Figure \ref{fig:reduction} describes a simple implementation of Consensus by $\Theta_{F,k=1}$. When a correct process $p_i$ invokes the {\sf propose}$(b)$ operation it loops invoking the {\sf getToken}$(b_0, b)$ operation as long as a valid block is eventually returned (lines \ref{r:while}-\ref{r:gettoken}). In this case the {\sf getToken}$()$ operation takes as input some block $b_0$ and the proposed block $b$. Afterwards, when the valid block has been obtained $p_i$ invokes the {\sf consumeToken}$(validBlock)$ operation whose result in stored in the $validBlockSet$ variable (line \ref{r:consumetoken}). Notice, the first process that invokes such operation is able to successfully consume the token, i.e., the valid block is in the Oracle set corresponding to $b_0$, which cardinality is $k=1$, and such set is returned each time the {\sf consumeToken}$()$ operation is invoked for a block related to $b_0$. Finally, (line \ref{r:decision}) the decision is triggered on such set (with contains one element) containing the element inserted by the first process that invoked the {\sf consumeToken}$()$ operation (the first write wins).

\begin{figure*}[t]
	\centering
	\fbox{
		\begin{minipage}{0.4\textwidth}
			%\footnotesize
			\scriptsize
			\resetline
			%\renewcommand{\baselinestretch}{2.5}
			\begin{tabbing}
				aaaA\=aA\=aA\=aaaA\kill
				
				%				{\bf Init}\\
				%				
				%				\line{} \> $validBlock \leftarrow \bot;$\\
				%				\line{} \> $validBlockSet \leftarrow \emptyset;$\\
				%				
				%				~-------------------------------------------------------\\
				
				{\bf upon event} ${\sf propose}(b)$:\\
				\line{} \> $validBlock \leftarrow \bot;$\\
				\line{} \> $validBlockSet \leftarrow \emptyset;$ \% since $k=1$ then it contains only one element. \\
				\line{r:while} \> {\bf while} $(validBlock = \bot)$: \\
				\line{r:gettoken} \>\>$validBlock \leftarrow \sf{getToken}(b_0, b)$;\\
				%\line{} \>{\bf endWhile} \\
				%\line{}\>\> $\dots$\\
				%\line{} \> $\dots$\\
				\line{r:consumetoken} \>$validBlockSet \leftarrow {\sf consumeToken}(validBlock)$; \% it can be different from validBlock\\
				\line{r:decision} \> {\bf trigger} {\sf decide}$(validBlockSet)$;\\
				%\line{} \> {\bf return}
				
				
			\end{tabbing}
			\normalsize
		\end{minipage}%
	}
	\caption{An implementation of Consensus by the Frugal Oracle with $k=1$.}
	\label{fig:reduction}   
\end{figure*}



\begin{theorem}\label{t:consensusOracleReduction}
	$\Theta_{F,k=1}$ Oracle has Consensus number $\infty$.
\end{theorem}


\subsubsection{Prodigal not stronger than an Atomic Register}

In order to show that the Prodigal oracle $\Theta_{P}$ has consensus number 1, it suffices to find a wait-free implementation of the oracle by an object with consensus number 1. To this end we present a straightforward implementation of the Prodigal oracle by Atomic Snapshot\cite{AH1990waitfree}. 

Let us firstly simplify the notation of the consume token operation. Let us consider a consume token invoked for a given block $b_h$, denoted as ${\sf consumeToken_h}(tkn_{m})$, which simply writes a token from the set $\mathfrak{T}=\{tkn_1,tkn_2, \dots, tkn_m,\dots\}$ in the set $K[h]$. Without loss of generality let us assume that: (i) tokens are  uniquely identified , (ii)  cardinality of $\mathfrak{T}$ is $n$ finite but not known and (iii) the set $K[h]$ is  represented by a collection of $n$ atomic registers $\mathfrak{K[h}=\{R_{h,1},R_{h,2}, \dots, R_{h,m},\dots R_{h,n}\}$, where $R_{h,m}$ is assigned to the $tkn_m$ token, i.e. $R_{h,m}$ can contain either $\bot$ or $tkn_m$. 

It can be observed that the  ${\sf consumeToken_h}(tkn_{m})$ in the case of $k$ infinite, always allows to write the token $tkn_{m}$ in $R_{h,m}$, i.e. there always exists a register $R_{h,m}$ for the proposed token $tkn_{m}$. By the oracle definition, moreover, the ${\sf consumeToken_h}(tkn_{m})$ returns a read of the $n$ registers that includes the last written token. Figure \ref{fig:CTtoAS} shows a  trivial implementation of commit token $CT$ using Atomic Snapshot that offers  ${\sf update}(R_i, value)$,  ${\sf scan}(R_1, R_2, \dots, R_n)$ operation to update a particular register and perform an atomic read of input registers, respectively. 

\begin{figure*}[t]
	\centering
	\fbox{
		\begin{minipage}{0.4\textwidth}
			%\footnotesize
			\scriptsize
			\resetline
			%\renewcommand{\baselinestretch}{2.5}
			\begin{tabbing}
				aaaA\=aA\=aA\=aaaA\kill
				\line{} {\sf consumeToken$_k$}$(tkn):$\\
				\line{}\> \> $R_{h,m}$ $\leftarrow${\sf update}$(R_{h,m}, tkn_m)$\\
				\line{} \>\>  $returned\_value \leftarrow {\sf scan(R_{h,1},R_{h,2}, \dots, R_{h,m},\dots R_{h,n})}$\\
				\line{}  \>\>{\bf return} $returned\_value$;\\
			\end{tabbing}
			\normalsize
		\end{minipage}	
	}
	\caption{An implementation of CT by Atomic Snapshot in the case of $\Theta_{P}$.}
	\label{fig:CTtoAS}   
\end{figure*}

\begin{theorem}\label{t:CTtoAS}
	$\Theta_{P}$ Oracle has Consensus number $1$.
\end{theorem}

\begin{proof}
	The proof trivially follows from  implementation  in Figure \ref{fig:CTtoAS}  of the consensus token operation of the Prodigal oracle by the Atomic Snaposhot object and from \cite{AH1990waitfree}. 
\end{proof}


\subsection{Implementability in a message-passing system model}

In this section we are interested in 
distributed message-passing implementations of BT-ADTs. More in detail we present \emph{(i)} the necessity of a light form of reliable broadcast to implement BT Eventual consistency,  \emph{(ii)}  refinement of BTs with Oracles that are not implementable in a message-passing system and \emph{(iii)} the mapping of current existing implementations with our abstract data types. 
%\subsection{Model of the system}
%\label{sec:blockch-syst-model}
To this end, we consider a message-passing system composed of an arbitrary large but finite set of $n$ processes that can be either Byzantine or correct. Each correct process of the distributed system executes a distributed protocol $\mathcal{P}$. A process is said to be Byzantine faulty if arbitrarily deviates from the protocol $\mathcal{P}$. %A Byzantine process is said to be faulty, otherwise it is correct. We make no assumption on the number of failures that can occur during the system execution. 
Processes communicate via message passing and the communication channels can be asynchronous or synchronous (see \cite{SDbook2011}), we specify each time the channels synchrony assumption considered, by default we consider asynchronous channels.
The BlockTree is now a shared object replicated at each process, we note by  $bt_i$ the local copy of the BlockTree maintained at  process $i$.
To maintain the replicated object we consider histories made of events related to the {\sf read}  and {\sf append}  operations on the shared object,  i.e. the {\sf send} and {\sf receive} operations for process communications and  the {\sf update} operation for BlockTree replica updates.  We also use subscript  $i$ to indicate that the operation occurred at process $i$: {\sf update}$_i(b_g,b_i$) indicates that $i$ inserts its locally generated valid block \emph{b}$_i$ in $bt_i$ with \emph{$b_g$} as a predecessor. Updates are communicated through {\sf send} and {\sf receive} operations. An update related to a block $b_i$ generated on a process $p_i$, sent through {\sf send}$_i(b_g,b_i)$, and received through a {\sf receive}$_j(b_g,b_i)$, takes effect on the local replica $bt_j$ of $p_j$ with the operation {\sf update}$_j(b_g,b_i)$. 



%In the remaining part of this work we consider implementations of BT-ADT  in a Byzantine failure model where the set of events $E$ is restricted to a countable set of events that contains \emph{(i)} all the BT-ADT  {\sf read}$()$ operations invocation events by the \emph{correct} processes,  \emph{(ii)} all BT-ADT {\sf read}$()$ operations response events at the \emph{correct} processes,  \emph{(iii)} all {\sf append}$(b)$ operations invocation events such that $b$ satisfies the predicate $P$ and,  \emph{(iv)} $send$, $receive$ and $update$ events generated at correct processes. Note that the Oracle-ADT is by construction agnostic to failures.


\subsubsection{Necessity of reliable communication}\label{par:comm-abstr} We define the properties on the communication primitives that each history $H$ generated by a BT-ADT satisfying the Eventual Prefix Property must satisfy. To this end we first introduce the following definition:

\begin{definition}[Update agreement]\label{def:historyUpdate}
	A concurrent history $H=\langle \Sigma, E, \Lambda, \mapsto, \prec, \nearrow \rangle$ generated by a BT-ADT satisfies the update agreement property if properties R1, R2 and R3 hold.
	\begin{itemize}
		\item R1. $\forall {\sf update}_i(b_g,b_i) \in H$, $\exists {\sf send}_i(b_g,b_i)\in H$;
		\item R2.  $\forall {\sf update}_i(b_g,b_j) \in H, \exists {\sf receive}_i(b_g,b_j) \in H$ such that ${\sf receive}_i(b_g,b_j) \mapsto {\sf update}_i(b_g,b_j)$;
		\item R3.  $\forall {\sf update}_i(b_g,b_j) \in H$, $\exists {\sf receive}_k(b_g,b_j)\in H, \forall k$.
	\end{itemize}
\end{definition}
%\setcounter{theorem}{2}
\begin{theorem}\label{th:updateAgreementNecessityEventualM}
	%	There does not exist concurrent historys $H=\langle \Sigma, E, \Lambda, \mapsto, \prec, \nearrow \rangle$ of the system generated by a BT-ADT that satisfies the Eventual BT Coherency criterion but not the Update Agreement.
	The update agreement property is necessary to construct concurrent histories $H=\langle \Sigma, E, \Lambda, \mapsto, \prec, \nearrow \rangle$ generated by a BT-ADT that satisfy the BT Eventual Consistency criterion.
\end{theorem}
For space reason the proof of the theorem can be found in \cite{BTADT2018TR}. The intuition behind the proof is that to meet BT Eventual Consistency all the processes must have the same view of BlockTree eventually. In fact missing an update on the branch that will be eventually selected (which cannot be a-priori-known) would imply that the prefix (which will be arbitrarily long) for the process that missed the update will diverge forever. 
Thanks to Theorem \ref{th:updateAgreementNecessityEventualM} we can finally prove  that the following communication primitive, inspired by \cite{SDbook2011} is  necessary to implement BT Eventual consistency :


\begin{definition}[Light Reliable Communication (LRC)]
	%The Light Reliable Communication abstraction satisfies the following properties:
	A concurrent history $H$ satisfies the properties of the LRC abstraction if and only if:
	\begin{itemize}
		\item (Validity): % If a correct process $i$ sends a message $m$ then $i$ eventually delivers $m$:
		$\forall {\sf send}_i(b,b_i) \in H, \exists {\sf receive}_i(b,b_i) \in H$;
		\item (Agreement): % If a message $m$ is delivered by  some correct process, them $m$ is eventually delivered by every correct process.
		$\forall {\sf receive}_i(b,b_j) \in H, \forall k \exists {\sf receive}_k(b,b_i) \in H$
	\end{itemize}
\end{definition}
The proof of the necessity is based on the necessity of Validity and Agreement for $R1, R2$ and $R3$. The interested reader can refer to \cite{BTADT2018TR} for the formal proof. 
\noindent
%In other words, a concurrent history $H$ satisfies the properties of the LRC abstraction if:
%\begin{itemize}
%	\item{LRC1.} $\forall {\sf send}_i(b,b_i) \in H, \exists {\sf deliver}_i(b,b_i) \in H$;
%	\item{LRC2.} $\forall {\sf deliver}_i(b,b_j) \in H, \forall k \exists {\sf deliver}_k(b,b_i) \in H$.
%\end{itemize} 


%
\begin{theorem}\label{th:LRCNecessity}
	The LRC abstraction is necessary for any BT-ADT implementation that generates concurrent histories that satisfies the BT Eventual Consistency criterion.
\end{theorem}

%\begin{corollary}\label{c:LRCNecessityStrong}
%	The LRC abstraction is necessary to for any BT-ADT implementation that generates concurrent histories that satisfies the BT Strong Consistency criterion.
%\end{corollary}
Let us note that, thanks to Theorem \ref{th:strongImpliesEventualM},  the results trivially hold for the BT Strong consistency criterion.

\subsubsection{Impossibility of BT Strong Consistency with forks}
%\{Impossibility results.}
\label{par:noforksstroing}
The following theorem states that BT Strong consistency cannot be implemented if forks can occur. Intuitively the proof is based on showing a scenario in which two concurrent updates $b_i$ and $b_j$ are issued, linked to a same block $b$ and two reads at two different processes read $b^{ \frown }b_i$ and $b^{ \frown }b_j$, violating the Strong prefix property. \\
\textbf{Observation.}
	Following our Oracle based abstraction (Section \ref{sec:bt-adt-augmented}) we assume by definition that the synchronization on the block to append is oracle side and takes place during the append operation. It follows that when a process takes the token to append a block it can only use the LRC communication abstraction.
%\setcounter{theorem}{4}
\begin{theorem}\label{t:noForkBeStrong}
	There does not exist an implementation of $\mathfrak{R}(\text{BT-ADT}_{ SC}, \Theta)$ with  $\Theta\neq \Theta_{F,k=1}$ that uses a LRC primitive and generates histories satisfying the BT Strong consistency.
\end{theorem}

The direct implication of the theorem is the non-implementability of refinement $\mathfrak{R}(\text{BT-ADT}_{ SC}, \Theta_{P})$ and $\mathfrak{R}(\text{BT-ADT}_{ SC}, \Theta_{F,k>1})$, in gray in Figure \ref{fig:BTHierarchyPurgedM}.

From Theorem \ref{t:noForkBeStrong} the next Corollary follows.
\begin{corollary}
	$\Theta_{F,k=1}$ is necessary for any implementation of any $\mathfrak{R}(\text{BT-ADT}_{ SC}, \Theta)$ that generates histories satisfying the BT Strong consistency.
\end{corollary}

Thanks to Theorem \ref{t:consensusOracleReduction} the next Corollary also follows.

\begin{corollary}
	Consensus is necessary for any implementation of a BT-ADT that generates histories satisfying the BT Strong consistency.
\end{corollary}

%\begin{lemma}\label{l:impossibilityAsynchr}
%	There does not exist an implementation of a BT-ADT refined with a $\Theta_P$-ADT that uses the LRC primitive and generates histories satisfying the BT Eventual consistency in an asynchronous communication system. 
%\end{lemma}
%
%\begin{lemma}\label{l:impossibilityTooManyBlocks}
%	There does not exist an implementation of a BT-ADT refined with a $\Theta_P$-ADT that uses the LRC primitive and generates histories satisfying the BT Eventual consistency in an synchronous communication system if the interval $T$ between the generation of two consecutive blocks is always smaller than $\delta$, the upper bound on message delay. 
%\end{lemma}

\subsection{Mapping with existing Blockchain implementations}
\label{sec:mapp-with-exist}


%\section{Mapping with existing Blockchain-like systems}
%\label{sec:mapp-with-exist}


We complete this work by illustrating the mapping in the following table between different existing systems and the specifications and abstractions presented in this paper. Interestingly, the mapping shows that all the proposed abstractions are implemented (even though in a probabilistic way in some case), and that the only two refinements used are $\mathfrak{R}(BT$-$ADT_{S C}, \Theta_{F,k=1})$ and $\mathfrak{R}(BT$-$ADT_{E C}, \Theta_P)$. In the following we discuss into details Bitcoin and Redbelly, an interested reader can find the discussions for the other systems in \cite{BTADT2018TR}.


\begin{table}[h]
	\centering
	\caption{Mapping of existing systems. Each of these systems assumes at least a light reliable communication.}
	\label{tab:mappingM}
	\begin{tabular}{llllll}
		References  &  Refinement \\
		\hline
		Bitcoin~\cite{bitcoin} & \(\mathfrak{R}(BT$-$ADT_{E C}, \Theta_P)\) \\
		Ethereum~\cite{Ethereum}  &  \(\mathfrak{R}(BT$-$ADT_{E C}, \Theta_P)\) \\
		Algorand~\cite{gilad2017algorand}  &  \(\mathfrak{R}(BT$-$ADT_{S C}, \Theta_{F,k=1})\) $SC$ w.h.p    \\
		ByzCoin~\cite{BizCoin}   &  \(\mathfrak{R}(BT$-$ADT_{S C}, \Theta_{F,k=1})\) \\
		PeerCensus~\cite{PeerCensus} & \(\mathfrak{R}(BT$-$ADT_{S C}, \Theta_{F,k=1})\)\\
		Redbelly~\cite{redbelly17}    &  \(\mathfrak{R}(BT$-$ADT_{S C},\Theta_{F,k=1})\) \\
		Hyperledger~\cite{HyperLedger} &  \(\mathfrak{R}(BT$-$ADT_{S C}, \Theta_{F,k=1})\)  \\
	\end{tabular}
\end{table}


 



\subsection{Bitcoin}
Bitcoin~\cite{bitcoin} is the pioneer of blockchain systems. Any process \(p\in V\) is allowed to {\sf read} the BlockTree and {\sf append} blocks to the BlockTree. Processes are characterized by their computational power represented by \(\alpha_p\), normalized as \(\sum_{p\in V}\alpha_p = 1\).   The  {\sf getToken} operation is implemented by a proof-of-work mechanism. The {\sf consumeToken} operation returns true for all valid blocks, thus there is no bounds on the number of consumed tokens. Thus Bitcoin implements a Prodigal Oracle.  The  \(f\) {\sf selects} returns the blockchain which has required the most computational work, guaranteeing that concurrent blocks can only refer to  the most recently appended blocks of the blockchain returned by a read() operation. Garay and al~\cite{GarayKL15} have shown, under a synchronous environment assumption, that Bitcoin ensures Eventual consistency criteria. The same conclusion applies as well for the FruitChain protocol \cite{PS17}, which proposes a protocol similar to BitCoin except for the rewarding mechanism.


\subsection{Red Belly}
Red Belly~\cite{redbelly17} is a consortium blockchain, meaning that any process \(p \in V\) is allowed to {\sf read} the BlockTree but a predefined subset \(M \subseteq V\) of processes are allowed to {\sf append} blocks. Each process \(p \in M\) as a merit parameter set to \(\alpha_p = 1/|M|\) while each process \(p \in V \setminus M\) has a merit parameter \(\alpha_p = 0\). %Processes are asynchronous (i.e.,  there is  no assumption on their respective computational speed) and are connected with partially synchronous~\cite{jacm88} (i.e., messages are delivered in unknown but finite time), reliable and authenticated communication channels. 
Each process \(p \in M\) can invoke the {\sf getToken} operation with their new block and will receive a token. The  {\sf consumeToken} operation, implemented by a Byzantine consensus algorithm run by all the processes in \(V\), returns true for the uniquely decided  block. 
Thus Red Belly  BlockTree  contains a unique blockchain, meaning that the selection function \(f\) is the trivial projection function from \(\mathcal{BT} \mapsto \mathcal{BC}\) which associates to the BT-ADT its unique existing chain of the BlockTree. As a consequence Red Belly relies on a Frugal Oracle with $k=1$, and by the properties of Byzantine agreement implements a  strongly consistent BlockTree (see Theorem 3~\cite{redbelly17}). 




%\begin{table}[h]
%	\centering
%	\caption{Mapping of existing systems. Each of these systems assumes at least a light reliable communication.\label{tab:mapping}}
%	\label{t:mapping}
%	\begin{tabular}{llllll}
%		References  & Permission &  Refinement & Consistency \\
%		\hline
%		Bitcoin~\cite{bitcoin}     &  no   & \(\mathfrak{R}(BT$-$ADT, \Theta_P)\)        & \(\Diamond C\) \\
%		Ethereum~\cite{Ethereum}     &  no      &  \(\mathfrak{R}(BT$-$ADT, \Theta_P)\)       &  \(\Diamond C\) \\
%		Algorand~\cite{Algorand2017}    &  no         &  \(\mathfrak{R}(BT$-$ADT, \Theta_{F,K=1})\)    & \(SC\) with v.h.p         \\
%		ByzCoin~\cite{BizCoin}     &  no    &  \(\mathfrak{R}(BT$-$ADT, \Theta_{F,K=1})\)   & \(SC\)          \\
%		PeerCensus~\cite{PeerCensus}  &  no   & \(\mathfrak{R}(BT$-$ADT, \Theta_{F,K=1})\)    & \(SC\)       \\
%		Redbelly~\cite{redbelly17}    &  yes   &  \(\mathfrak{R}(BT$-$ADT, \Theta_{F,K=1})\)  & \(SC\)                    \\
%		Hyperledger~\cite{HyperLedger} &  yes  &  \(\mathfrak{R}(BT$-$ADT, \Theta_{F,K=1})\)          & \(SC\)                 \\
%	\end{tabular}
%\end{table}

 



==> discussion.tex <==
% !TeX root = main.tex


We present the BlockTree specifications varying the the Oracle employed, and Prefix property, letting the other properties fixed. To such purpose we employ such notation: ({Oracle}, {Prefix Convergence property})-BT. From the reasoning in Section \ref{ssec:oracleHierarchy} we can consider directly only two different types of Generate Validity, denoted as  Forkable and Fork-free. From the combination of Oracle and Prefix properties we derive the hierarchy depicted in the Figure \ref{fig:BTHierarchy} in which the case $(Forkable,Strong)-BT$ does not exist. Let us consider the scenario depicted in Figure \ref{fig:forkNoStrong}. If forks can occur then the Strong prefix property can not be guaranteed.
\AD{Aiming for an Eventual prefix semantic is better to use a Forkable Oracle, having a Fork-free Oracle it is easy to have a Strong semantic, so the middle level BT is not so interesting.}

{\color{red}
\begin{itemize}
	\item forkable $\Rightarrow$ no strong prefix (cf. figure);
	\item Asynchrony $\vee$ Permissionless $\Rightarrow$ no Consensus $\Rightarrow$ forkable;
	\item no reliable broadcast $\Rightarrow$ no append termination $\Rightarrow$ no eventual prefix;
	\item Permissionless (unbounded churn) $\Rightarrow$ no reliable broadcast $\Rightarrow$ no append termination $\Rightarrow$ no strong prefix.
\end{itemize}
}

\begin{figure}
	\begin{tikzpicture}[scale=0.7]
	\node[] () at (-2,1) {$\mathcal{F}(BT^{t}_{j})$};
	\node [circle,draw,thick] (0j) at (0,1) {$b_{0,-}$};
	\node [circle,draw] (1i) at (2,2) {$b_{1,j}$};	
	\node [circle,draw] (3i) at (4,2) {$b_{2,j}$};
	\node [circle,draw, gray!30] (2i) at (2,0) {$b_{1,i}$};							
	\draw[<-]
	(0j) edge (1i) (1i) edge (3i)  ;
	
	\draw[<-,gray!30] (0j) edge (2i);
	
	\draw[-] (-1,-1) -- (5,-1);
	
	\node[] () at (-2,-3) {$\mathcal{F}(BT^{t}_{i})$};			
	\node [circle,draw,thick] (0i) at (0,-3) {$b_{0,-}$};
	\node [circle,draw] (2) at (2,-4) {$b_{1,i}$};					
	\node [circle,draw] (4) at (4,-4) {$b_{2,i}$};
	\node [circle,draw, gray!30] (1j) at (2,-2) {$b_{1,j}$};			
	\draw[<-]
	(0i) edge (2) (2) edge (4) 
	;
	
	\draw[<-,gray!30] (0i) edge (1j);
	\end{tikzpicture}\caption{$(Forkable,Strong)-BT$ Scenario in which all the node appended after the genesis node are countercurrently appended to a {\sf read}$()$ operation in which $\mathcal()$ returns the longest chain. In such case $v_i$ and $v_j$ read different branches violating the Strong Prefix property. }  \label{fig:forkNoStrong}
\end{figure}


\begin{figure}
	\begin{tikzpicture}[scale=0.7]
	\node[] () at (-2,1) {$\mathcal{F}(BT^{t}_{j})$};
	\node [circle,draw,thick] (0j) at (0,1) {$b_{0,-}$};
	\node [circle,draw] (1i) at (2,1) {$b_{1,j}$};	
	\node [circle,draw] (3i) at (4,1) {$b_{2,j}$};						
	\draw[<-]
	(0j) edge (1i) (1i) edge (3i)  ;
	
	
	\draw[-] (-1,-1) -- (5,-1);
	
	\node[] () at (-2,-3) {$\mathcal{F}(BT^{t}_{i})$};			
	\node [circle,draw,thick] (0i) at (0,-3) {$b_{0,-}$};
	\node [circle,draw] (2) at (2,-3) {$b_{1,j}$};					
	\draw[<-]
	(0i) edge (2)
	;
	
	\end{tikzpicture}\caption{$(Fork-free),\diamondsuit)-BT$ Scenario that respect the Eventual Prefix property. In such case $h=1$.}  \label{fig:NoforkStrong}
\end{figure}


\begin{figure}
	\begin{tikzpicture}
	
	\node[draw](1) at (0,0) {$(Fork-free),Strong)-BT$};
	\node[draw](2) at (-3,-2) {$(Fork-free),\diamondsuit)-BT$};
	
	\node[draw, gray!40](3) at (3,-2) {$(Forkable,Strong)-BT$};
	\node[draw](4) at (0,-4) {$(Forkable,\diamondsuit)-BT$};
	
	\draw[->, gray!30]
	(1) edge (3)
	(3) edge (4)  
	;
	
	\draw[->] (1) edge (4) (1) edge (2) (2) edge (4) ;
	
	\draw[->] (-5.2,1)--(-5.2,-5); \node[rotate=90] () at (-5.5,-3) {Weaker BT properties};				
	\end{tikzpicture}
	\caption{BT Hierarchy. }\label{fig:BTHierarchy}
\end{figure}


==> intro.tex <==

Blockchain technology became today one of the most appealing area of research motivated mainly by its huge potential in the design of a broad class of secured distributed applications. The volume of transactions that are reported every day in Bitcoin \cite{bitcoin} for example is 218,000 for a value of 400,000,000\$ in average and is continuing increasing. Blockchain systems maintain a continuously-growing history of ordered blocks, each block being composed of transactions\footnote{Transaction is used here as a generic name to be adapted to a broad class of use cases. For example, a transaction in Bitcoin \cite{bitcoin} or Ethereum \cite{Ethereum} can be a transfer of digital money or assets.} that have been verified by the members of the system, called miners.  Blocks are linked to each other by relying on hash functions and  the order of blocks in the blockchain is the result of a form of agreement among the system participants. At any time, participants strongly agree on a prefix of the blockchain, the suffix of the blockchain being potentially different at participants.% (see Figure \ref{blockchain}). 
 
%  \begin{figure}[h]
% \begin{center}
% \includegraphics[scale=0.4]{blockchain-mini}
% \end{center}
% \caption{\label{blockchain} \bf{Bitcoin's blockchain.}}
% \end{figure}

%Emmanuelle: I removed this sentence because this is an incident due to programming issues. This is not due to a misconception of Ethereum
%Blockchain systems, beyond their incontestable assets such as decentralization, simple design and relative easy-to-use,  are not free of incidents and limitations. The most popular incident  reported for Ethereum for example was the 60 million dollars ether theft which was possible by simply exploiting an error in the code and the lack of system specification.  

 
A recent study~\cite{KonigW16} has shown that despite their large adoption  blockchains are far from being a  \say{ready-to-use} technology in critical economical applications and scientists multiply their efforts in warning about the risks of using this technology before understanding and fully mastering it. 
%which has focused on several limitations of the most popular blockchain, Bitcoin including weak security,  low quality of service, storage limitations, low throughput, high cost and weak coherency, 
%Moreover, popular blockchains claim that they totally linearize transactions by implementing consensus in a asynchronous  dynamic open system. This claim is refuted by the famous impossibility result in traditional distributing computing \cite{FLP}. 
%
%Interestingly, many recent attempts to alarm on vulnerabilities  of popular blockchains are target of defenders brigading. 
Nevertheless, we are convinced that once fully mastered, Blockchain-based systems will be the technical solution for fully decentralized activities that were for centuries centralized such as administration and banking. Blockchain may unlock new application scenarios in several sectors such as energy, health, food, etc. especially in conjunction with IoTs and artificial intelligence. Such applications have various consistency and quality of service requirements, advocating for a family of blockchains.
 
 In this respect we are interested in formalizing the blockchains as a family of formal specifications that can be combined to meet specific consistency criteria.  To this end we provide specifications as a composition of \emph{abstract data types} together with a hierarchy of \emph{consistency criteria} that formally characterizes the histories admissibles for distributed programs that use them. The advantage of specifying shared objects as abstract data types over implementation-based alternatives such as~\cite{GGGHS17} is the possibility to reason on the consistency of a system independently of the communication model~\cite{perrin:hal-01286755}.
%
More precisely, we define two abstract data types, the \emph{BlockTree} and the \emph{Oracle}. The BlockTree models the blockchain data structure, which is a tree of blocks providing an \emph{append} and a \emph{read} operation. The append operation is intended to insert a new leaf in the tree, provided that the newly inserted block is valid.  The validity property of a block in the BlockTree is abstracted as a general predicate, which is implementation specific. For instance, in Bitcoin a valid block is a block containing a hash $hs$ of three fields: the field containing the set of in-block transactions, the hash of the previous block, and a nonce (proof-of-work) such that the resulting hash $hs$ starts with a given number of leading zeros.

 In our formalisation, what makes a block valid, i.e. triggering the validity predicate at true, is indeed the \emph{Oracle}.  The Oracle abstracts the mechanism used to grant processes the insertion of new blocks in the blockchain, such as proof of work or other agreement mechanisms. To this end the Oracle is modeled as a simple token manager. We say that a token is generated when a process obtains the right to extend a given block in the chain with a new valid block, and we say that a token is consumed once the process successfully extends the chain.


\textit{The composition of the BlockTree and the Oracle fully specify a blockchain.} Indeed, admissible histories of BlockTree only contain executions of append operations appending valid blocks, where  validity is conditional to the oracle behavior. 

\textbf{Sara: Work in progress.....}
Let us note that it would have been possible to abstract a blockchain only through the BlockTree abstract data type, hiding then the validity predicate by embedding the validation process in the implementation of the append operation. We advocate that the separation of the blockchain in two different abstractions, however, has several benefits.  

The first advantage is the possibility to deal with liveness properties at finer granularity level, separating the termination of the validation process, managed by the Oracle, from the termination of updating a replicated data structure, managed by the BlockTree.  That separation is very useful  since in many implementations the Oracle is a probabilistic local process, while the  process of updating a replicated data structure relies on reliable update diffusion and some local deterministic rule to eventually converge on the same totally ordered set of updates. It has been noted that in those implementations the fact the the Oracle is probabilistic does not necessarily imply that the BlockTree is propabilistic per-se, it is indeed the composition that is probabilistic and in particular the composed liveness properties. 

As for safety properties, the separation allows to properly deal with the notion of validity. As it has been noted in  \cite{} a valid block indeed is always \say{admissible},  even if sent by a byzantine process. This notion of validity can then be captured  to properly define the problem of updating a replicated data structure with valid data, solely managed by the BlockTree. 


Furthermore, the possibility to reason on the BlockTree in isolation, allowed us to extend the consistency criteria theory with a new consistency criterion for BlockTree that captures the eventual convergence process in blockchain systems. We introduce in this respect a weaker consistency criterion than the so-called monotonic prefix consistency criterion, introduced in~\cite{GGGHS17}. The monotonic prefix consistency criterion informally says that any two reads return two chains such that one is the prefix of the other. We indeed relax this consistency criterion admitting any two chains to have a divergent prefix for a finite interval of the history, defining then the \emph{Eventual Prefix} property. Note that we also define a so-called \emph{Strong Prefix} property that is equivalent, under certain conditions, to  the monotonic prefix consistency criterion.  In the end, we define  two BlockTree versions, one enjoying the Eventual Prefix property and the other one enjoying the Strong Prefix property. The two versions are called \textit{Eventual BlockTree} and \textit{Strong Block Tree}, respectively. 

The oracle  enjoys two different versions as well. The weakest one is an oracle \say{without memory}, called \emph{Prodigal} and the other is an oracle \say{with memory}, called \emph{Frugal}. The Prodigal Oracle, without memory, does not remember how many tokens it provided for a given block to extend, while the Frugal oracle counts the number of tokens provided and the ones actually consumed for any block. In practical terms, the Prodigal oracle  does not control the number of forks in the system, while the Frugal oracle embeds mechanisms to restrict the number of forks up to $k$. 

Given those specifications we formally show the necessary conditions that must hold on the communication model to implement the BlockTree with Eventual Prefix in a message-passing system. Interestingly, we show the necessity of a light form of reliable broadcast enjoying both the Validity (if  a correct process sends a message then it eventually delivers it) and Agreement (if a message is delivered by some correct process then the message is eventually delivered by every correct process) properties. 

We finally map our specifications to existing representative blockchains. We show that RedBelly is an implementation of  a Strong BlockTree composed with a Frugal Oracle,  Algorand is a propabilistic implementation of a Strong BlockTree composed with an Frugal Oracle, while BitCoin is a probabilistic implementation of an Eventual BlockTree composed with a Prodigal Oracle. 





 
%
%Interestingly, our abstract data types are designed to be easily integrated in  libraries such as CODS \cite{matthiew-thesis} specifically designed for implementing distributed shared objects with various levels of consistency. 


%
%
% 
%In \cite{GGGHS17} the authors prove that monotonic prefix consistency criterion is the strongest criterion implementable in systems prone to partitions. Then they show that the monotonic prefix consistency is implemented by Bitcoin.
% 
% 
%\paragraph{Related work.}
%\subsection{State of the art} 

%The birth of blockchains systems, as for the case of P2P systems in the early 2000, was in the non academic research.
%After the releasing of the most popular blockchains  (e.g. Bitcoin \cite{bitcoin} or Ethereum \cite{Ethereum}) with a specific focus on economical transactions their huge potential  for various other applications became evident.  
%However, quickly after their release blockchains reached their limits in terms of throughput, blocksize and unforeseen behaviors. Therefore, 
%non academic research further concentrate in  proposing alternatives by improving some  performance aspects but with non zero costs either on security or throughput. 
%  
% On the academic side many studies have been dedicated in the last ten years to the  \emph{security and privacy} aspects in blockchains.   
%
%
%%\subsection{Agreement in blockchains}
%Interestingly, only recently distributed computing scientist started to investigate theoretical aspects of blockchains and several directions of research can be identified: blockchains based on \emph{proof-of-work}(the power of block building is proportional to the computational power of nodes) and its alternatives such as \emph{proof-of-stake}(the power of block building is proportional to the amount of money nodes own in the system),  \emph{proof-of-space} or \emph{proof-of-authority} (the power of block building is proportional to the amount of authority nodes own in the system), blockchains using as underlying building block the achievements in classical \emph{practical Byzantine fault-tolerance} and finally \emph{sortition} based blockchains.   
%
%The theoretical study of \emph{proof-of-work} based blockchains has been  pioneered by Garay et \emph{al}~\cite{GarayKL15}.   Garay et \emph{al} decorticate the pseudo-code of Bitcoin and  analyze its agreement aspects considering a synchronous round-based communication model. That is, messages sent in a round are assumed to arrive in the next round. This study  has been extended by Pass et \emph{al}~\cite{PSS17}  to round based systems where messages sent in a round can be received later. The major criticisms for the \emph{proof-of-work} approach are as follows: it is assumed that the honest miners hold a majority of the computational power, the generation of a block is energetically costly which yielded to the creation of mining pools and finally, the multiple blockchains that coexist in the system.  
% 
%In order to overcome the drawbacks of Bicoin, \cite{Bitcoin-NG} proposes a mix between proof-of-work blockchains and proof-of-work free blockchains referred as Bitcoin-NG. The idea is that the execution of the system is organized in epochs. In each epoch a leader elected via a proof-of-work mechanism will decide the order transactions that will be committed in the blockchain till the next epoch. Bitcoin-NG inherits the drawbacks of Bitcoin: costly proof-of-work process, forks, no guarantee that a leader in an epoch is unique, no guarantee that the leader do not change the history at will if the leader is corrupted.
%
%Recently, \cite{BizCoin} propose an alternative to the proof-of-work based blockchains, named Byzcoin. Their research build on top of \emph{practical Byzantine fault-tolerance} \cite{pbft}  enhanced with a scalable collective signing process.   \cite{BizCoin} is based on a leader-based consensus over a group of members chosen based on a proof-of-membership mechanism. As in Bitcoin, when a miner succeeds to mine a block it is included in the voting members set that excludes one member. This protocol also inherits some of the Bitcoin problems and vulnerabilities. Also Byzcoin voting core can be totally corrupted by a dynamic adversary.  
%
%In order to avoid some of the previously cited problems,  Micali~\cite{micali2016} introduced (further extended in \cite{BPS16, micali2017a})
%the \emph{sortition} based blockchains that completely replace the proof-of-work mechanism by sortition.  These works focus again the  agreement aspects of blockchains using probabilistic ingredients. More specifically, the set of nodes that are allowed to produce and validate blocks are randomly chosen and they change over the time. Interestingly, the study focuses only on synchronous round-based communication models which do not  reflect the reality of blockchain technologies. 
%
%
%In another line of research, Pass \emph{et al.} address in \cite{PS17}   one of the vulnerabilities of Bitcoin studied formally in Eyal and Sirer \cite{ES14} (if the adversary controls a coalition of miners holding even a  minority fraction of the computational power, this coalition can gain twice its share). 
  

%  \emph{Decker et al.} \cite{PeerCensus} opened the line of research related to the coherency of blockchains. They propose PeerCensus system that targets to provide the linearizability of transactions. PeerCensus combines, similar to Byzcoin,  the proof-of-work blockchain and the classical results in practical byzantine agreement fault tolerance. PeerCensus suffers of the same drawbacks as Bitcoin and Byzcoin face to dynamic adversaries. Also, the exact level of coherency ensured by PeerCensus is not yet formally proven.  
%
%The recent work of \cite{ALPT17} makes the connection between the Bitcoin blockchain and the shared registered theory proving that the the Bitcoin system offers a coherency equivalent to the regular register. In \cite{GGGHS17} the authors prove that monotonic prefix consistency criterion is the strongest criterion implementable in systems prone to partitions. Then they show that the monotonic prefix consistency is implemented by Bitcoin. 




 
%\paragraph{Our contribution.}




%%% Local Variables:
%%% coding: utf-8
%%% mode: latex
%%% TeX-master: "main.tex"
%%% ispell-local-dictionary: "english"
%%% End:


==> paper.tex <==
% !TeX root = main.tex

==> related.tex <==
% !TeX root = main.tex

Bitcoin~\cite{bitcoin} is considered as the pioneer cryptocurrency systems. Since its inception, several altcoins~\cite{altcoins} have emerged. Most of their differences lie in practical details like use of a database~\cite{namecoin}, block generation time~\cite{Ethereum}, used hashing algorithm~\cite{litecoin} or an unlimited number of coins~\cite{peercoin}.
%
The GHOST protocol~\cite{GHOST} proposes a different rule to solve blockchain forks, based on the number of blocks contained in each blockchain subtree (in case of consecutive forks).
Meanwhile, CoinJoin~\cite{CoinJoin} and CoinShuffle~\cite{CoinShuffle} propose to mix transactions to avoid user linkability. 
Recent works have focused on Bitcoin modeling and evaluation.
Authors of~\cite{bitcoinmodel} prove that the Bitcoin protocol achieves consensus with high probability, while~\cite{GarayKL15} show that peers participating in the Bitcoin network agree on a common prefix for the transaction history,
 both in
failure-free environments. 
In contrast, authors of~\cite{KAC2012, KARGC2015} focused on adversarial environments. These works study the feasibility  of double spending attacks and 
their detection.
%


In~\cite{bitcoinng}, authors proposed to rely on a natural leader election provided by blocks appended in the blockchain to serialize all transactions issued in the system under leader's watch. In the current setting, a leader has thus to sign and serialize in average 1500 transactions per block. This volume is steadily growing, leading to question about scalability of this approach.
%%
Approach~\cite{PeerCensus} proposes a off-chain record to impose strong consistency. In addition to analysis studied in Section~\ref{sec:strongc}, this approach shared the scalability flaw of~\cite{bitcoinng}~: byzantine resilient state machine replication usually rely on a leader, proposing operations to a quorum for validation. This kind of approach~\cite{PBFT99, Zyzzyva07,  Aliph10} barely scale beyond 10 participants.

In the following, we will present a deep analysis of these cryptosystems.
\AD{to discuss: the guerraoui paper about lists, prefixes, blockchain and the coq paper.}
% !TeX root = mainV3.tex
